Object-based reasoning in VQA

Visual Question Answering (VQA) is a novel problem domain where multi-modal inputs must be processed in order to solve the task given in the form of a natural language. As the solutions inherently require to combine visual and natural language processing with abstract reasoning, the problem is considered as AI-complete. Recent advances indicate that using high-level, abstract facts extracted from the inputs might facilitate reasoning. Following that direction we decided to develop a solution combining state-of-the-art object detection and reasoning modules. The results, achieved on the well-balanced CLEVR dataset, confirm the promises and show significant, few percent improvements of accuracy on the complex "counting" task.

==> img/scheme_answer_decoding.sla.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<SCRIBUSUTF8NEW Version="1.4.3.svn">
    <DOCUMENT ANZPAGES="1" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" PRESET="0" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" ORIENTATION="1" PAGESIZE="A4" FIRSTNUM="1" BOOK="0" AUTOSPALTEN="1" ABSTSPALTEN="11" UNITS="0" DFONT="Abyssinica SIL Regular" DSIZE="12" DCOL="1" DGAP="0" TabFill="" TabWidth="36" AUTHOR="" COMMENTS="" KEYWORDS="" PUBLISHER="" DOCDATE="" DOCTYPE="" DOCFORMAT="" DOCIDENT="" DOCSOURCE="" DOCLANGINFO="" DOCRELATION="" DOCCOVER="" DOCRIGHTS="" DOCCONTRIB="" TITLE="" SUBJECT="" VHOCH="33" VHOCHSC="66" VTIEF="33" VTIEFSC="66" VKAPIT="75" BASEGRID="5" BASEO="0" AUTOL="20" UnderlinePos="-1" UnderlineWidth="-1" StrikeThruPos="-1" StrikeThruWidth="-1" GROUPC="2" HCMS="0" DPSo="0" DPSFo="0" DPuse="0" DPgam="0" DPbla="1" DPMo="CineonLog M " DPPr="Fogra27L CMYK Coated Press" DPIn="CineonLog M " DPInCMYK="Fogra27L CMYK Coated Press" DPIn2="CineonLog M " DPIn3="Fogra27L CMYK Coated Press" DISc="1" DIIm="0" ALAYER="0" LANGUAGE="English" MINWORDLEN="3" HYCOUNT="2" AUTOMATIC="1" AUTOCHECK="0" GUIDELOCK="0" SnapToGuides="0" SnapToGrid="0" MINGRID="10" MAJGRID="10" SHOWGRID="0" SHOWGUIDES="0" showcolborders="1" SHOWFRAME="0" SHOWLAYERM="0" SHOWMARGIN="0" SHOWBASE="0" SHOWPICT="1" SHOWControl="0" SHOWLINK="0" rulerMode="0" showrulers="0" showBleed="0" rulerXoffset="100" rulerYoffset="20" GuideRad="10" GRAB="4" POLYC="4" POLYF="0.707" POLYR="0" POLYCUR="0" POLYFD="0" POLYS="0" AutoSave="1" AutoSaveTime="600000" ScratchBottom="20" ScratchLeft="100" ScratchRight="100" ScratchTop="20" GapHorizontal="0" GapVertical="40" StartArrow="0" EndArrow="0" PEN="Black" BRUSH="None" PENLINE="Black" PENTEXT="Black" StrokeText="Black" TextBackGround="None" TextLineColor="None" TextBackGroundShade="100" TextLineShade="100" TextPenShade="100" TextStrokeShade="100" STIL="1" STILLINE="1" WIDTH="1" WIDTHLINE="1" PENSHADE="100" LINESHADE="100" BRUSHSHADE="100" MAGMIN="10" MAGMAX="3200" MAGSTEP="200" CPICT="None" PICTSHADE="100" PICTSCX="1" PICTSCY="1" PSCALE="1" PASPECT="1" EmbeddedPath="0" HalfRes="1" dispX="10" dispY="10" constrain="15" MINORC="#aa0000" MAJORC="#aa0000" GuideC="#000080" BaseC="#c0c0c0" GuideZ="10" BACKG="1" PAGEC="#ffffff" MARGC="#0000ff" RANDF="0" currentProfile="PostScript">
        <CheckProfile Name="PDF 1.3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.4" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.5" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF/X-3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="1" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PostScript" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <COLOR NAME="Black" CMYK="#000000ff" Spot="0" Register="0"/>
        <COLOR NAME="Blue" RGB="#0000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cool Black" CMYK="#990000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cyan" CMYK="#ff000000" Spot="0" Register="0"/>
        <COLOR NAME="FromEPS#00000070" CMYK="#00000070" Spot="0" Register="0"/>
        <COLOR NAME="Green" RGB="#00ff00" Spot="0" Register="0"/>
        <COLOR NAME="Grey58" RGB="#949494" Spot="0" Register="0"/>
        <COLOR NAME="Magenta" CMYK="#00ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Red" RGB="#ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Registration" CMYK="#ffffffff" Spot="0" Register="1"/>
        <COLOR NAME="Rich Black" CMYK="#996666ff" Spot="0" Register="0"/>
        <COLOR NAME="Snow2" RGB="#eee9e9" Spot="0" Register="0"/>
        <COLOR NAME="Snow4" RGB="#8b8989" Spot="0" Register="0"/>
        <COLOR NAME="Warm Black" CMYK="#00994cff" Spot="0" Register="0"/>
        <COLOR NAME="White" CMYK="#00000000" Spot="0" Register="0"/>
        <COLOR NAME="Yellow" CMYK="#0000ff00" Spot="0" Register="0"/>
        <HYPHEN/>
        <STYLE NAME="Default Paragraph Style" DefaultStyle="1" ALIGN="0" LINESPMode="0" LINESP="15" INDENT="0" RMARGIN="0" FIRST="0" VOR="0" NACH="0" DROP="0" DROPLIN="2" DROPDIST="0"/>
        <CHARSTYLE CNAME="Default Character Style" DefaultStyle="1" FONT="Abyssinica SIL Regular" FONTSIZE="12" FEATURES="inherit" FCOLOR="Black" FSHADE="100" SCOLOR="Black" SSHADE="100" TXTSHX="5" TXTSHY="-5" TXTOUT="1" TXTULP="-0.1" TXTULW="-0.1" TXTSTP="-0.1" TXTSTW="-0.1" SCALEH="100" SCALEV="100" BASEO="0" KERN="0" LANGUAGE="English"/>
        <LAYERS NUMMER="0" LEVEL="0" NAME="Background" SICHTBAR="1" DRUCKEN="1" EDIT="1" FLOW="1" TRANS="1" BLEND="0" OUTL="0" LAYERC="#000000"/>
        <Printer firstUse="1" toFile="1" useAltPrintCommand="1" outputSeparations="1" useSpotColors="0" useColor="0" mirrorH="0" mirrorV="0" useICC="0" doGCR="0" doClip="0" setDevParam="0" useDocBleeds="0" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" includePDFMarks="0" PSLevel="3" PDLanguage="3" markOffset="6.94181282764193e-310" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" printer="" filename="" separationName="" printerCommand=""/>
        <PDF firstUse="0" Thumbnails="0" Articles="0" Bookmarks="0" Compress="1" CMethod="0" Quality="0" MirrorH="0" MirrorV="0" Clip="0" RotateDeg="0" PresentMode="0" RecalcPic="0" Grayscale="0" RGBMode="1" UseProfiles="0" UseProfiles2="0" Binding="0" PicRes="300" Resolution="300" Version="14" Intent="1" Intent2="0" SolidP="CineonLog M " ImageP="CineonLog M " PrintP="Fogra27L CMYK Coated Press" InfoString="" BTop="0" BLeft="0" BRight="0" BBottom="0" useDocBleeds="1" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" docInfoMarks="0" markOffset="0" ImagePr="0" PassOwner="" PassUser="" Permissions="-4" Encrypt="0" UseLayers="0" UseLpi="0" UseSpotColors="1" doMultiFile="0" displayBookmarks="0" displayFullscreen="0" displayLayers="0" displayThumbs="0" hideMenuBar="0" hideToolBar="0" fitWindow="0" PageLayout="0" openAction="">
            <Fonts Name="Abyssinica SIL Regular"/>
            <Effekte pageEffectDuration="1" pageViewDuration="1" effectType="0" Dm="0" M="0" Di="0"/>
            <LPI Color="" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Black" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Cyan" Frequency="133" Angle="105" SpotFunction="3"/>
            <LPI Color="Magenta" Frequency="133" Angle="75" SpotFunction="3"/>
            <LPI Color="Yellow" Frequency="133" Angle="90" SpotFunction="3"/>
        </PDF>
        <DocItemAttributes/>
        <TablesOfContents/>
        <PageSets>
            <Set Name="Single Page" FirstPage="0" Rows="1" Columns="1"/>
            <Set Name="Double Sided" FirstPage="1" Rows="1" Columns="2">
                <PageNames Name="Left Page"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="3-Fold" FirstPage="0" Rows="1" Columns="3">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="4-Fold" FirstPage="0" Rows="1" Columns="4">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle Left"/>
                <PageNames Name="Middle Right"/>
                <PageNames Name="Right Page"/>
            </Set>
        </PageSets>
        <Sections>
            <Section Number="0" Name="0" From="0" To="0" Type="Type_1_2_3" Start="1" Reversed="0" Active="1"/>
        </Sections>
        <MASTERPAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="Normal" MNAM="" Size="A4" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="280" PAGEHEIGHT="50" BORDERLEFT="38" BORDERRIGHT="0" BORDERTOP="10" BORDERBOTTOM="40" NUM="0" NAM="" MNAM="Normal" Size="Custom" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="83" YPOS="33" WIDTH="45" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_ar^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="125" YPOS="43" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="149" YPOS="30" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="147" YPOS="28" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="211" YPOS="24" WIDTH="45" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$a^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="230" YPOS="43" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="254" YPOS="30" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="252" YPOS="28" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="148" YPOS="35" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="MLP"/>
            <para/>
            <ITEXT CH="(Softmax)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="156.5" YPOS="31.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="162.5" YPOS="31.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="156.453125" YPOS="32.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="162.453125" YPOS="32.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="162.453125" YPOS="32.09375" WIDTH="11.6943496" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="138.9004937" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="156.453125" YPOS="32.09375" WIDTH="11.62821276" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="41.07728711" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="152" YPOS="41" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="158" YPOS="41" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="164" YPOS="41" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="155" YPOS="34" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="161" YPOS="34" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="335" YPOS="43" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="335" YPOS="34" WIDTH="45" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$y^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="105" YPOS="52" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Blue" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="252" YPOS="35" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="Word"/>
            <para/>
            <ITEXT CH="decoding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
    </DOCUMENT>
</SCRIBUSUTF8NEW>


==> img/scheme_general.sla.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<SCRIBUSUTF8NEW Version="1.4.3.svn">
    <DOCUMENT ANZPAGES="1" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" PRESET="0" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" ORIENTATION="1" PAGESIZE="A4" FIRSTNUM="1" BOOK="0" AUTOSPALTEN="1" ABSTSPALTEN="11" UNITS="0" DFONT="Abyssinica SIL Regular" DSIZE="12" DCOL="1" DGAP="0" TabFill="" TabWidth="36" AUTHOR="" COMMENTS="" KEYWORDS="" PUBLISHER="" DOCDATE="" DOCTYPE="" DOCFORMAT="" DOCIDENT="" DOCSOURCE="" DOCLANGINFO="" DOCRELATION="" DOCCOVER="" DOCRIGHTS="" DOCCONTRIB="" TITLE="" SUBJECT="" VHOCH="33" VHOCHSC="66" VTIEF="33" VTIEFSC="66" VKAPIT="75" BASEGRID="5" BASEO="0" AUTOL="20" UnderlinePos="-1" UnderlineWidth="-1" StrikeThruPos="-1" StrikeThruWidth="-1" GROUPC="1" HCMS="0" DPSo="0" DPSFo="0" DPuse="0" DPgam="0" DPbla="1" DPMo="CineonLog M " DPPr="Fogra27L CMYK Coated Press" DPIn="CineonLog M " DPInCMYK="Fogra27L CMYK Coated Press" DPIn2="CineonLog M " DPIn3="Fogra27L CMYK Coated Press" DISc="1" DIIm="0" ALAYER="0" LANGUAGE="English" MINWORDLEN="3" HYCOUNT="2" AUTOMATIC="1" AUTOCHECK="0" GUIDELOCK="0" SnapToGuides="0" SnapToGrid="0" MINGRID="10" MAJGRID="10" SHOWGRID="0" SHOWGUIDES="0" showcolborders="1" SHOWFRAME="0" SHOWLAYERM="0" SHOWMARGIN="0" SHOWBASE="0" SHOWPICT="1" SHOWControl="0" SHOWLINK="0" rulerMode="0" showrulers="0" showBleed="0" rulerXoffset="100" rulerYoffset="20" GuideRad="10" GRAB="4" POLYC="4" POLYF="0.707" POLYR="0" POLYCUR="0" POLYFD="0" POLYS="0" AutoSave="1" AutoSaveTime="600000" ScratchBottom="20" ScratchLeft="100" ScratchRight="100" ScratchTop="20" GapHorizontal="0" GapVertical="40" StartArrow="0" EndArrow="0" PEN="Black" BRUSH="None" PENLINE="Black" PENTEXT="Black" StrokeText="Black" TextBackGround="None" TextLineColor="None" TextBackGroundShade="100" TextLineShade="100" TextPenShade="100" TextStrokeShade="100" STIL="1" STILLINE="1" WIDTH="1" WIDTHLINE="1" PENSHADE="100" LINESHADE="100" BRUSHSHADE="100" MAGMIN="10" MAGMAX="3200" MAGSTEP="200" CPICT="None" PICTSHADE="100" PICTSCX="1" PICTSCY="1" PSCALE="1" PASPECT="1" EmbeddedPath="0" HalfRes="1" dispX="10" dispY="10" constrain="15" MINORC="#aa0000" MAJORC="#aa0000" GuideC="#000080" BaseC="#c0c0c0" GuideZ="10" BACKG="1" PAGEC="#ffffff" MARGC="#0000ff" RANDF="0" currentProfile="PostScript">
        <CheckProfile Name="PDF 1.3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.4" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.5" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF/X-3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="1" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PostScript" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <COLOR NAME="Black" CMYK="#000000ff" Spot="0" Register="0"/>
        <COLOR NAME="Blue" RGB="#0000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cool Black" CMYK="#990000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cyan" CMYK="#ff000000" Spot="0" Register="0"/>
        <COLOR NAME="FromEPS#00000070" CMYK="#00000070" Spot="0" Register="0"/>
        <COLOR NAME="Green" RGB="#00ff00" Spot="0" Register="0"/>
        <COLOR NAME="Grey58" RGB="#949494" Spot="0" Register="0"/>
        <COLOR NAME="Magenta" CMYK="#00ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Red" RGB="#ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Registration" CMYK="#ffffffff" Spot="0" Register="1"/>
        <COLOR NAME="Rich Black" CMYK="#996666ff" Spot="0" Register="0"/>
        <COLOR NAME="Snow2" RGB="#eee9e9" Spot="0" Register="0"/>
        <COLOR NAME="Snow4" RGB="#8b8989" Spot="0" Register="0"/>
        <COLOR NAME="Warm Black" CMYK="#00994cff" Spot="0" Register="0"/>
        <COLOR NAME="White" CMYK="#00000000" Spot="0" Register="0"/>
        <COLOR NAME="Yellow" CMYK="#0000ff00" Spot="0" Register="0"/>
        <HYPHEN/>
        <STYLE NAME="Default Paragraph Style" DefaultStyle="1" ALIGN="0" LINESPMode="0" LINESP="15" INDENT="0" RMARGIN="0" FIRST="0" VOR="0" NACH="0" DROP="0" DROPLIN="2" DROPDIST="0"/>
        <CHARSTYLE CNAME="Default Character Style" DefaultStyle="1" FONT="Abyssinica SIL Regular" FONTSIZE="12" FEATURES="inherit" FCOLOR="Black" FSHADE="100" SCOLOR="Black" SSHADE="100" TXTSHX="5" TXTSHY="-5" TXTOUT="1" TXTULP="-0.1" TXTULW="-0.1" TXTSTP="-0.1" TXTSTW="-0.1" SCALEH="100" SCALEV="100" BASEO="0" KERN="0" LANGUAGE="English"/>
        <LAYERS NUMMER="0" LEVEL="0" NAME="Background" SICHTBAR="1" DRUCKEN="1" EDIT="1" FLOW="1" TRANS="1" BLEND="0" OUTL="0" LAYERC="#000000"/>
        <Printer firstUse="1" toFile="1" useAltPrintCommand="1" outputSeparations="1" useSpotColors="0" useColor="0" mirrorH="0" mirrorV="0" useICC="0" doGCR="0" doClip="0" setDevParam="0" useDocBleeds="0" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" includePDFMarks="0" PSLevel="3" PDLanguage="3" markOffset="6.94181282764193e-310" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" printer="" filename="" separationName="" printerCommand=""/>
        <PDF firstUse="0" Thumbnails="0" Articles="0" Bookmarks="0" Compress="1" CMethod="0" Quality="0" MirrorH="0" MirrorV="0" Clip="0" RotateDeg="0" PresentMode="0" RecalcPic="0" Grayscale="0" RGBMode="1" UseProfiles="0" UseProfiles2="0" Binding="0" PicRes="300" Resolution="300" Version="14" Intent="1" Intent2="0" SolidP="CineonLog M " ImageP="CineonLog M " PrintP="Fogra27L CMYK Coated Press" InfoString="" BTop="0" BLeft="0" BRight="0" BBottom="0" useDocBleeds="1" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" docInfoMarks="0" markOffset="0" ImagePr="0" PassOwner="" PassUser="" Permissions="-4" Encrypt="0" UseLayers="0" UseLpi="0" UseSpotColors="1" doMultiFile="0" displayBookmarks="0" displayFullscreen="0" displayLayers="0" displayThumbs="0" hideMenuBar="0" hideToolBar="0" fitWindow="0" PageLayout="0" openAction="">
            <Fonts Name="Abyssinica SIL Regular"/>
            <Effekte pageEffectDuration="1" pageViewDuration="1" effectType="0" Dm="0" M="0" Di="0"/>
            <LPI Color="" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Black" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Cyan" Frequency="133" Angle="105" SpotFunction="3"/>
            <LPI Color="Magenta" Frequency="133" Angle="75" SpotFunction="3"/>
            <LPI Color="Yellow" Frequency="133" Angle="90" SpotFunction="3"/>
        </PDF>
        <DocItemAttributes/>
        <TablesOfContents/>
        <PageSets>
            <Set Name="Single Page" FirstPage="0" Rows="1" Columns="1"/>
            <Set Name="Double Sided" FirstPage="1" Rows="1" Columns="2">
                <PageNames Name="Left Page"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="3-Fold" FirstPage="0" Rows="1" Columns="3">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="4-Fold" FirstPage="0" Rows="1" Columns="4">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle Left"/>
                <PageNames Name="Middle Right"/>
                <PageNames Name="Right Page"/>
            </Set>
        </PageSets>
        <Sections>
            <Section Number="0" Name="0" From="0" To="0" Type="Type_1_2_3" Start="1" Reversed="0" Active="1"/>
        </Sections>
        <MASTERPAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="Normal" MNAM="" Size="A4" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="185" PAGEHEIGHT="85" BORDERLEFT="38" BORDERRIGHT="0" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="" MNAM="Normal" Size="Custom" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="101" YPOS="35" WIDTH="31.25" HEIGHT="21" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0651041666666667" LOCALSCY="0.0651041666666667" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 31.25 0 31.25 0 31.25 0 31.25 0 31.25 21 31.25 21 31.25 21 31.25 21 0 21 0 21 0 21 0 21 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 31.25 0 31.25 0 31.25 0 31.25 0 31.25 21 31.25 21 31.25 21 31.25 21 0 21 0 21 0 21 0 21 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="100" YPOS="71" WIDTH="32" HEIGHT="14.6875" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LINESPMode="1" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 32 0 32 0 32 0 32 0 32 14.6875 32 14.6875 32 14.6875 32 14.6875 0 14.6875 0 14.6875 0 14.6875 0 14.6875 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 32 0 32 0 32 0 32 0 32 14.6875 32 14.6875 32 14.6875 32 14.6875 0 14.6875 0 14.6875 0 14.6875 0 14.6875 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="What is the size of the object left of the brown cylinder?"/>
            <trail LINESPMode="1" LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="137" YPOS="27" WIDTH="52" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 5 0 5 0 0 0 0 0 0 0 0 52 0 52 0 52 0 52 0 52 5 52 5 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 53.43 0.1875 53.43 0.1875 53.43 0.1875 53.43 0.1875 53.43 7.3125 53.43 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="137" YPOS="21" WIDTH="52" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 7 52 7 52 7 52 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 7 52 7 52 7 52 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Image encoder"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="137" YPOS="88" WIDTH="52" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 0 0 0 0 5 0 5 0 5 0 5 52 5 52 5 52 5 52 5 52 0 52 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 53.43 0.1875 53.43 0.1875 53.43 0.1875 53.43 0.1875 53.43 7.3125 53.43 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="137" YPOS="95" WIDTH="52" HEIGHT="13" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 13 52 13 52 13 52 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 13 52 13 52 13 52 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Question encoder"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="192" YPOS="88" WIDTH="54" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 0 0 0 0 5 0 5 0 5 0 5 54 5 54 5 54 5 54 5 54 0 54 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 55.485 0.1875 55.485 0.1875 55.485 0.1875 55.485 0.1875 55.485 7.3125 55.485 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="190" YPOS="95" WIDTH="58.56" HEIGHT="13" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 58.56 0 58.56 0 58.56 0 58.56 0 58.56 13 58.56 13 58.56 13 58.56 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 58.56 0 58.56 0 58.56 0 58.56 0 58.56 13 58.56 13 58.56 13 58.56 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Semantic embedding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="249" YPOS="88" WIDTH="20" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 0 0 0 0 5 0 5 0 5 0 5 20 5 20 5 20 5 20 5 20 0 20 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 20.55 0.1875 20.55 0.1875 20.55 0.1875 20.55 0.1875 20.55 7.3125 20.55 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="245" YPOS="95" WIDTH="30" HEIGHT="13" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LINESPMode="1" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 13 30 13 30 13 30 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 13 30 13 30 13 30 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Answer"/>
            <para LINESPMode="1" LINESP="5"/>
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="decoder"/>
            <trail LINESPMode="1" LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="190" YPOS="58" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="193.333333333333" YPOS="58" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="3.33333333333334" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="196.666666666667" YPOS="58" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="6.66666666666666" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="197.333333333333" YPOS="65" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="3.33333333333334" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="200.666666666667" YPOS="65" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="6.66666666666666" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="194" YPOS="65" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="192" YPOS="62" WIDTH="10" HEIGHT="3" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="6" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="6" CH="..."/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="188" YPOS="55" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="191.333333333333" YPOS="55" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="3.33333333333334" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="194.666666666667" YPOS="55" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="6.66666666666666" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="182" YPOS="71" WIDTH="12" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="8" POCOOR="0 5 0 5 12 5 12 5 12 5 12 5 12 0 12 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 7.3125 12.33 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="182" YPOS="45" WIDTH="12" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="8" POCOOR="0 0 0 0 12 0 12 0 12 0 12 0 12 5 12 5 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 7.3125 12.33 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="182" YPOS="79" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="133" YPOS="45" WIDTH="4" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="153" YPOS="45" WIDTH="13" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="199" YPOS="56" WIDTH="5.92564606182318" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="333.705209929417" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="201" YPOS="59" WIDTH="4.68541620349788" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="350.788973459184" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="205" YPOS="66" WIDTH="5.14933248101155" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="5.57219780396389" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="219.875" YPOS="52.625" WIDTH="8.35410545169317" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="29.2116292191861" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="222.125" YPOS="58.4375" WIDTH="5.79321803192837" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="22.6394934193111" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="133" YPOS="76" WIDTH="4" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="153" YPOS="76" WIDTH="13" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="242.9" YPOS="61" WIDTH="8" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="266.9" YPOS="61" WIDTH="4" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="267.9" YPOS="60" WIDTH="20" HEIGHT="6" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" TXTFILL="Black" TXTFILLSH="100" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 20 0 20 0 20 0 20 0 20 6 20 6 20 6 20 6 0 6 0 6 0 6 0 6 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 20 0 20 0 20 0 20 0 20 6 20 6 20 6 20 6 0 6 0 6 0 6 0 6 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" FEATURES="inherit" FCOLOR="Black" FSHADE="100" CH="large"/>
            <trail ALIGN="1" LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="101" YPOS="21" WIDTH="30" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Image"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="101" YPOS="95" WIDTH="30" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Question"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="263" YPOS="95" WIDTH="30" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Answer"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="211" YPOS="62" WIDTH="10" HEIGHT="3" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="6" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="6" CH="..."/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="153" YPOS="79" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="154" YPOS="80" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="155" YPOS="81" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="156" YPOS="82" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.2" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="157" YPOS="83" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="182" YPOS="37" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="183" YPOS="38" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="184" YPOS="39" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="185" YPOS="40" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.2" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="186" YPOS="41" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="141" YPOS="35" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="140" YPOS="34" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="170" YPOS="35" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="169" YPOS="34" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="141" YPOS="56" WIDTH="22" HEIGHT="10" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Object"/>
            <para LINESP="3"/>
            <ITEXT FONTSIZE="3" CH="detection"/>
            <para/>
            <ITEXT CH="(Faster R-CNN)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="170" YPOS="66" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="169" YPOS="65" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="141" YPOS="66" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="140" YPOS="65" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="255" YPOS="51" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="254" YPOS="50" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="141" YPOS="87" WIDTH="22" HEIGHT="10" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Word"/>
            <para/>
            <ITEXT FONTSIZE="3" CH="embedding"/>
            <para/>
            <ITEXT FONTSIZE="3" CH="(GLOVE)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="172" YPOS="56" WIDTH="22" HEIGHT="10" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Object"/>
            <para LINESP="3"/>
            <ITEXT CH="Encoding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="231" YPOS="51" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="230" YPOS="50" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="234" YPOS="72" WIDTH="22" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 4 22 4 22 4 22 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 4 22 4 22 4 22 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Aggregation"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="256.9" YPOS="72" WIDTH="22" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 8 22 8 22 8 22 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 8 22 8 22 8 22 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <para/>
            <ITEXT CH="(Softmax)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="208" YPOS="50" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="207" YPOS="49" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="207" YPOS="50" WIDTH="11" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="210" YPOS="56" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="209" YPOS="55" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="209" YPOS="56" WIDTH="11" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="214" YPOS="65" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="213" YPOS="64" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="213" YPOS="65" WIDTH="11" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="225.75" YPOS="66.375" WIDTH="2.24" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="332.4471884" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="170" YPOS="87" WIDTH="22" HEIGHT="10" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Sentence"/>
            <para/>
            <ITEXT CH="encoding"/>
            <para/>
            <ITEXT CH="(LSTM)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="156" YPOS="35" WIDTH="3.25000000000004" HEIGHT="11.6308262887688" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0485074626865678" LOCALSCY="0.0485074626865678" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object1.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 11.6308 3.25 11.6308 3.25 11.6308 3.25 11.6308 0 11.6308 0 11.6308 0 11.6308 0 11.6308 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 11.6308 3.25 11.6308 3.25 11.6308 3.25 11.6308 0 11.6308 0 11.6308 0 11.6308 0 11.6308 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="7.31250000000003" gHeight="23.1875" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="156.8125" YPOS="35.9971744666635" WIDTH="3.25000000000004" HEIGHT="10.8272312416753" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0373563218390809" LOCALSCY="0.0373563218390809" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object2.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 10.8272 3.25 10.8272 3.25 10.8272 3.25 10.8272 0 10.8272 0 10.8272 0 10.8272 0 10.8272 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 10.8272 3.25 10.8272 3.25 10.8272 3.25 10.8272 0 10.8272 0 10.8272 0 10.8272 0 10.8272 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0.812500000000028" gYpos="2.99717446666353" gWidth="7.31250000000003" gHeight="23.1875" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="157.625" YPOS="37.5661811523752" WIDTH="3.25000000000004" HEIGHT="8.86382423683745" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0570175438596498" LOCALSCY="0.0570175438596498" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object3.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.86382 3.25 8.86382 3.25 8.86382 3.25 8.86382 0 8.86382 0 8.86382 0 8.86382 0 8.86382 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.86382 3.25 8.86382 3.25 8.86382 3.25 8.86382 0 8.86382 0 8.86382 0 8.86382 0 8.86382 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="1.625" gYpos="5.56618115237518" gWidth="7.31250000000003" gHeight="23.1875" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="158.4375" YPOS="38.5633556190387" WIDTH="3.25000000000004" HEIGHT="8.45495871330868" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0411392405063296" LOCALSCY="0.0411392405063296" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object4.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.45496 3.25 8.45496 3.25 8.45496 3.25 8.45496 0 8.45496 0 8.45496 0 8.45496 0 8.45496 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.45496 3.25 8.45496 3.25 8.45496 3.25 8.45496 0 8.45496 0 8.45496 0 8.45496 0 8.45496 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="2.43750000000001" gYpos="8.5633556190387" gWidth="7.31250000000003" gHeight="23.1875" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="159.25" YPOS="39.5605300857022" WIDTH="3.25000000000004" HEIGHT="8.43924901691914" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0471014492753629" LOCALSCY="0.0471014492753629" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object5.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.43925 3.25 8.43925 3.25 8.43925 3.25 8.43925 0 8.43925 0 8.43925 0 8.43925 0 8.43925 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.43925 3.25 8.43925 3.25 8.43925 3.25 8.43925 0 8.43925 0 8.43925 0 8.43925 0 8.43925 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="3.25000000000009" gYpos="11.5605300857022" gWidth="7.31250000000003" gHeight="23.1875" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="160.0625" YPOS="40.7717884428418" WIDTH="3.25000000000004" HEIGHT="8.41571155715824" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0560344827586214" LOCALSCY="0.0560344827586214" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object6.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.41571 3.25 8.41571 3.25 8.41571 3.25 8.41571 0 8.41571 0 8.41571 0 8.41571 0 8.41571 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.25 0 3.25 0 3.25 0 3.25 0 3.25 8.41571 3.25 8.41571 3.25 8.41571 3.25 8.41571 0 8.41571 0 8.41571 0 8.41571 0 8.41571 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="4.0625" gYpos="14.7717884428418" gWidth="7.31250000000003" gHeight="23.1875" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="243" YPOS="63" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Blue" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
    </DOCUMENT>
</SCRIBUSUTF8NEW>


==> img/scheme_general_scene_description.sla.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<SCRIBUSUTF8NEW Version="1.4.3.svn">
    <DOCUMENT ANZPAGES="1" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" PRESET="0" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" ORIENTATION="1" PAGESIZE="A4" FIRSTNUM="1" BOOK="0" AUTOSPALTEN="1" ABSTSPALTEN="11" UNITS="0" DFONT="Abyssinica SIL Regular" DSIZE="12" DCOL="1" DGAP="0" TabFill="" TabWidth="36" AUTHOR="" COMMENTS="" KEYWORDS="" PUBLISHER="" DOCDATE="" DOCTYPE="" DOCFORMAT="" DOCIDENT="" DOCSOURCE="" DOCLANGINFO="" DOCRELATION="" DOCCOVER="" DOCRIGHTS="" DOCCONTRIB="" TITLE="" SUBJECT="" VHOCH="33" VHOCHSC="66" VTIEF="33" VTIEFSC="66" VKAPIT="75" BASEGRID="5" BASEO="0" AUTOL="20" UnderlinePos="-1" UnderlineWidth="-1" StrikeThruPos="-1" StrikeThruWidth="-1" GROUPC="1" HCMS="0" DPSo="0" DPSFo="0" DPuse="0" DPgam="0" DPbla="1" DPMo="CineonLog M " DPPr="Fogra27L CMYK Coated Press" DPIn="CineonLog M " DPInCMYK="Fogra27L CMYK Coated Press" DPIn2="CineonLog M " DPIn3="Fogra27L CMYK Coated Press" DISc="1" DIIm="0" ALAYER="0" LANGUAGE="English" MINWORDLEN="3" HYCOUNT="2" AUTOMATIC="1" AUTOCHECK="0" GUIDELOCK="0" SnapToGuides="0" SnapToGrid="0" MINGRID="10" MAJGRID="10" SHOWGRID="0" SHOWGUIDES="0" showcolborders="1" SHOWFRAME="0" SHOWLAYERM="0" SHOWMARGIN="0" SHOWBASE="0" SHOWPICT="1" SHOWControl="0" SHOWLINK="0" rulerMode="0" showrulers="0" showBleed="0" rulerXoffset="100" rulerYoffset="20" GuideRad="10" GRAB="4" POLYC="4" POLYF="0.707" POLYR="0" POLYCUR="0" POLYFD="0" POLYS="0" AutoSave="1" AutoSaveTime="600000" ScratchBottom="20" ScratchLeft="100" ScratchRight="100" ScratchTop="20" GapHorizontal="0" GapVertical="40" StartArrow="0" EndArrow="0" PEN="Black" BRUSH="None" PENLINE="Black" PENTEXT="Black" StrokeText="Black" TextBackGround="None" TextLineColor="None" TextBackGroundShade="100" TextLineShade="100" TextPenShade="100" TextStrokeShade="100" STIL="1" STILLINE="1" WIDTH="1" WIDTHLINE="1" PENSHADE="100" LINESHADE="100" BRUSHSHADE="100" MAGMIN="10" MAGMAX="3200" MAGSTEP="200" CPICT="None" PICTSHADE="100" PICTSCX="1" PICTSCY="1" PSCALE="1" PASPECT="1" EmbeddedPath="0" HalfRes="1" dispX="10" dispY="10" constrain="15" MINORC="#aa0000" MAJORC="#aa0000" GuideC="#000080" BaseC="#c0c0c0" GuideZ="10" BACKG="1" PAGEC="#ffffff" MARGC="#0000ff" RANDF="0" currentProfile="PostScript">
        <CheckProfile Name="PDF 1.3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.4" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.5" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF/X-3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="1" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PostScript" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <COLOR NAME="Black" CMYK="#000000ff" Spot="0" Register="0"/>
        <COLOR NAME="Blue" RGB="#0000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cool Black" CMYK="#990000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cyan" CMYK="#ff000000" Spot="0" Register="0"/>
        <COLOR NAME="FromEPS#00000070" CMYK="#00000070" Spot="0" Register="0"/>
        <COLOR NAME="Green" RGB="#00ff00" Spot="0" Register="0"/>
        <COLOR NAME="Grey58" RGB="#949494" Spot="0" Register="0"/>
        <COLOR NAME="Magenta" CMYK="#00ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Red" RGB="#ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Registration" CMYK="#ffffffff" Spot="0" Register="1"/>
        <COLOR NAME="Rich Black" CMYK="#996666ff" Spot="0" Register="0"/>
        <COLOR NAME="Snow2" RGB="#eee9e9" Spot="0" Register="0"/>
        <COLOR NAME="Snow4" RGB="#8b8989" Spot="0" Register="0"/>
        <COLOR NAME="Warm Black" CMYK="#00994cff" Spot="0" Register="0"/>
        <COLOR NAME="White" CMYK="#00000000" Spot="0" Register="0"/>
        <COLOR NAME="Yellow" CMYK="#0000ff00" Spot="0" Register="0"/>
        <HYPHEN/>
        <STYLE NAME="Default Paragraph Style" DefaultStyle="1" ALIGN="0" LINESPMode="0" LINESP="15" INDENT="0" RMARGIN="0" FIRST="0" VOR="0" NACH="0" DROP="0" DROPLIN="2" DROPDIST="0"/>
        <CHARSTYLE CNAME="Default Character Style" DefaultStyle="1" FONT="Abyssinica SIL Regular" FONTSIZE="12" FEATURES="inherit" FCOLOR="Black" FSHADE="100" SCOLOR="Black" SSHADE="100" TXTSHX="5" TXTSHY="-5" TXTOUT="1" TXTULP="-0.1" TXTULW="-0.1" TXTSTP="-0.1" TXTSTW="-0.1" SCALEH="100" SCALEV="100" BASEO="0" KERN="0" LANGUAGE="English"/>
        <LAYERS NUMMER="0" LEVEL="0" NAME="Background" SICHTBAR="1" DRUCKEN="1" EDIT="1" FLOW="1" TRANS="1" BLEND="0" OUTL="0" LAYERC="#000000"/>
        <Printer firstUse="1" toFile="1" useAltPrintCommand="1" outputSeparations="1" useSpotColors="0" useColor="0" mirrorH="0" mirrorV="0" useICC="0" doGCR="0" doClip="0" setDevParam="0" useDocBleeds="0" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" includePDFMarks="0" PSLevel="3" PDLanguage="3" markOffset="6.94181282764193e-310" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" printer="" filename="" separationName="" printerCommand=""/>
        <PDF firstUse="0" Thumbnails="0" Articles="0" Bookmarks="0" Compress="1" CMethod="0" Quality="0" MirrorH="0" MirrorV="0" Clip="0" RotateDeg="0" PresentMode="0" RecalcPic="0" Grayscale="0" RGBMode="1" UseProfiles="0" UseProfiles2="0" Binding="0" PicRes="300" Resolution="300" Version="14" Intent="1" Intent2="0" SolidP="CineonLog M " ImageP="CineonLog M " PrintP="Fogra27L CMYK Coated Press" InfoString="" BTop="0" BLeft="0" BRight="0" BBottom="0" useDocBleeds="1" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" docInfoMarks="0" markOffset="0" ImagePr="0" PassOwner="" PassUser="" Permissions="-4" Encrypt="0" UseLayers="0" UseLpi="0" UseSpotColors="1" doMultiFile="0" displayBookmarks="0" displayFullscreen="0" displayLayers="0" displayThumbs="0" hideMenuBar="0" hideToolBar="0" fitWindow="0" PageLayout="0" openAction="">
            <Fonts Name="Abyssinica SIL Regular"/>
            <Effekte pageEffectDuration="1" pageViewDuration="1" effectType="0" Dm="0" M="0" Di="0"/>
            <LPI Color="" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Black" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Cyan" Frequency="133" Angle="105" SpotFunction="3"/>
            <LPI Color="Magenta" Frequency="133" Angle="75" SpotFunction="3"/>
            <LPI Color="Yellow" Frequency="133" Angle="90" SpotFunction="3"/>
        </PDF>
        <DocItemAttributes/>
        <TablesOfContents/>
        <PageSets>
            <Set Name="Single Page" FirstPage="0" Rows="1" Columns="1"/>
            <Set Name="Double Sided" FirstPage="1" Rows="1" Columns="2">
                <PageNames Name="Left Page"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="3-Fold" FirstPage="0" Rows="1" Columns="3">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="4-Fold" FirstPage="0" Rows="1" Columns="4">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle Left"/>
                <PageNames Name="Middle Right"/>
                <PageNames Name="Right Page"/>
            </Set>
        </PageSets>
        <Sections>
            <Section Number="0" Name="0" From="0" To="0" Type="Type_1_2_3" Start="1" Reversed="0" Active="1"/>
        </Sections>
        <MASTERPAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="Normal" MNAM="" Size="A4" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="185" PAGEHEIGHT="85" BORDERLEFT="38" BORDERRIGHT="0" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="" MNAM="Normal" Size="Custom" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="100" YPOS="71" WIDTH="32" HEIGHT="14.6875" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LINESPMode="1" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 32 0 32 0 32 0 32 0 32 14.6875 32 14.6875 32 14.6875 32 14.6875 0 14.6875 0 14.6875 0 14.6875 0 14.6875 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 32 0 32 0 32 0 32 0 32 14.6875 32 14.6875 32 14.6875 32 14.6875 0 14.6875 0 14.6875 0 14.6875 0 14.6875 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="What is the size of the object left of the brown cylinder?"/>
            <trail LINESPMode="1" LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="137" YPOS="88" WIDTH="52" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 0 0 0 0 5 0 5 0 5 0 5 52 5 52 5 52 5 52 5 52 0 52 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 53.43 0.1875 53.43 0.1875 53.43 0.1875 53.43 0.1875 53.43 7.3125 53.43 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="137" YPOS="95" WIDTH="52" HEIGHT="13" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 13 52 13 52 13 52 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 13 52 13 52 13 52 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Question encoder"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="192" YPOS="88" WIDTH="54" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 0 0 0 0 5 0 5 0 5 0 5 54 5 54 5 54 5 54 5 54 0 54 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 55.485 0.1875 55.485 0.1875 55.485 0.1875 55.485 0.1875 55.485 7.3125 55.485 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="190" YPOS="95" WIDTH="58.56" HEIGHT="13" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 58.56 0 58.56 0 58.56 0 58.56 0 58.56 13 58.56 13 58.56 13 58.56 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 58.56 0 58.56 0 58.56 0 58.56 0 58.56 13 58.56 13 58.56 13 58.56 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Semantic embedding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="249" YPOS="88" WIDTH="20" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 0 0 0 0 5 0 5 0 5 0 5 20 5 20 5 20 5 20 5 20 0 20 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 20.55 0.1875 20.55 0.1875 20.55 0.1875 20.55 0.1875 20.55 7.3125 20.55 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="245" YPOS="95" WIDTH="30" HEIGHT="13" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LINESPMode="1" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 13 30 13 30 13 30 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 13 30 13 30 13 30 13 0 13 0 13 0 13 0 13 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Answer"/>
            <para LINESPMode="1" LINESP="5"/>
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="decoder"/>
            <trail LINESPMode="1" LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="190" YPOS="58" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="193.333333333333" YPOS="58" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="3.33333333333334" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="196.666666666667" YPOS="58" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="6.66666666666666" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="197.333333333333" YPOS="65" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="3.33333333333334" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="200.666666666667" YPOS="65" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="6.66666666666666" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="194" YPOS="65" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="192" YPOS="62" WIDTH="10" HEIGHT="3" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="6" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="6" CH="..."/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="188" YPOS="55" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="191.333333333333" YPOS="55" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="3.33333333333334" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="194.666666666667" YPOS="55" WIDTH="3.33333333333333" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 3.33333 0 3.33333 0 3.33333 0 3.33333 0 3.33333 2 3.33333 2 3.33333 2 3.33333 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="6.66666666666666" gYpos="0" gWidth="10" gHeight="2" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="182" YPOS="71" WIDTH="12" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="8" POCOOR="0 5 0 5 12 5 12 5 12 5 12 5 12 0 12 0 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 7.3125 12.33 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="182" YPOS="45" WIDTH="12" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="8" POCOOR="0 0 0 0 12 0 12 0 12 0 12 0 12 5 12 5 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 0.1875 12.33 7.3125 12.33 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="182" YPOS="79" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.5" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="199" YPOS="56" WIDTH="5.92564606182318" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="333.705209929417" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="201" YPOS="59" WIDTH="4.68541620349788" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="350.788973459184" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="205" YPOS="66" WIDTH="5.14933248101155" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="5.57219780396389" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="219.875" YPOS="52.625" WIDTH="8.35410545169317" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="29.2116292191861" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="222.125" YPOS="58.4375" WIDTH="5.79321803192837" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="22.6394934193111" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="133" YPOS="76" WIDTH="4" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="153" YPOS="76" WIDTH="13" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="242.9" YPOS="61" WIDTH="8" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="266.9" YPOS="61" WIDTH="4" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="267.9" YPOS="60" WIDTH="20" HEIGHT="6" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" TXTFILL="Black" TXTFILLSH="100" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 20 0 20 0 20 0 20 0 20 6 20 6 20 6 20 6 0 6 0 6 0 6 0 6 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 20 0 20 0 20 0 20 0 20 6 20 6 20 6 20 6 0 6 0 6 0 6 0 6 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" FEATURES="inherit" FCOLOR="Black" FSHADE="100" CH="large"/>
            <trail ALIGN="1" LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="101" YPOS="95" WIDTH="30" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Question"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="263" YPOS="95" WIDTH="30" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 7 30 7 30 7 30 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Answer"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="211" YPOS="62" WIDTH="10" HEIGHT="3" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="6" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 3 10 3 10 3 10 3 0 3 0 3 0 3 0 3 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="6" CH="..."/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="153" YPOS="79" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="154" YPOS="80" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="155" YPOS="81" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="156" YPOS="82" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.2" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="157" YPOS="83" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="182" YPOS="37" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="183" YPOS="38" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="184" YPOS="39" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="185" YPOS="40" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.2" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="186" YPOS="41" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="170" YPOS="66" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="169" YPOS="65" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="141" YPOS="66" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="140" YPOS="65" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="255" YPOS="51" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="254" YPOS="50" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="141" YPOS="87" WIDTH="22" HEIGHT="10" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Word"/>
            <para/>
            <ITEXT FONTSIZE="3" CH="embedding"/>
            <para/>
            <ITEXT FONTSIZE="3" CH="(GLOVE)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="231" YPOS="51" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="230" YPOS="50" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="234" YPOS="72" WIDTH="22" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 4 22 4 22 4 22 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 4 22 4 22 4 22 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Aggregation"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="256.9" YPOS="72" WIDTH="22" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 8 22 8 22 8 22 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 8 22 8 22 8 22 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <para/>
            <ITEXT CH="(Softmax)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="208" YPOS="50" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="207" YPOS="49" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="207" YPOS="50" WIDTH="11" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="210" YPOS="56" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="209" YPOS="55" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="209" YPOS="56" WIDTH="11" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="214" YPOS="65" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="213" YPOS="64" WIDTH="11" HEIGHT="5" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 3 11 3 11 3 11 4.10457 9 5 10.1046 5 9 5 9 5 2 5 2 5 2 5 0.895431 5 0 3 0 4.10457 0 3 0 3 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="213" YPOS="65" WIDTH="11" HEIGHT="4" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 11 0 11 0 11 0 11 0 11 4 11 4 11 4 11 4 0 4 0 4 0 4 0 4 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="225.75" YPOS="66.375" WIDTH="2.24" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="332.4471884" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="170" YPOS="87" WIDTH="22" HEIGHT="10" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="3" CH="Sentence"/>
            <para/>
            <ITEXT CH="encoding"/>
            <para/>
            <ITEXT CH="(LSTM)"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="243" YPOS="63" WIDTH="10" HEIGHT="2" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Blue" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 10 0 10 0 10 0 10 0 10 2 10 2 10 2 10 2 0 2 0 2 0 2 0 2 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="7" XPOS="163.75" YPOS="28" WIDTH="25.25" HEIGHT="5" RADRECT="0" FRTYPE="3" CLIPEDIT="1" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="12" POCOOR="0 5 0 5 0 0 0 0 0 0 0 0 25.25 0 25.25 0 25.25 0 25.25 0 25.25 5 25.25 5 " NUMCO="12" COCOOR="0 4.875 0 4.875 0 0 0 0 0 0 0 0 25.9444 0.1875 25.9444 0.1875 25.9444 0.1875 25.9444 0.1875 25.9444 7.3125 25.9444 7.3125 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="149" YPOS="22" WIDTH="52" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 7 52 7 52 7 52 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 52 0 52 0 52 0 52 0 52 7 52 7 52 7 52 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Scene encoder"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="96" YPOS="22" WIDTH="54" HEIGHT="7" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="5" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="4" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 54 0 54 0 54 0 54 0 54 7 54 7 54 7 54 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 54 0 54 0 54 0 54 0 54 7 54 7 54 7 54 7 0 7 0 7 0 7 0 7 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="4" CH="Scene description"/>
            <trail LINESP="5"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="170" YPOS="36" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="169" YPOS="35" WIDTH="11" HEIGHT="22" RADRECT="2" FRTYPE="2" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMCO="32" COCOOR="2 0 2 0 9 0 9 0 9 0 10.1046 0 11 2 11 0.895431 11 2 11 2 11 20 11 20 11 20 11 21.1046 9 22 10.1046 22 9 22 9 22 2 22 2 22 2 22 0.895431 22 0 20 0 21.1046 0 20 0 20 0 2 0 2 0 2 0 0.895431 2 0 0.895431 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="170" YPOS="57" WIDTH="22" HEIGHT="10" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="3" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 22 0 22 0 22 0 22 0 22 10 22 10 22 10 22 10 0 10 0 10 0 10 0 10 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="Scene"/>
            <para/>
            <ITEXT CH="description"/>
            <para/>
            <ITEXT CH="encoding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="99" YPOS="36.8125" WIDTH="60.6875" HEIGHT="26.8125" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESPMode="1" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" ISIZE="3" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 60.6875 0 60.6875 0 60.6875 0 60.6875 0 60.6875 26.8125 60.6875 26.8125 60.6875 26.8125 60.6875 26.8125 0 26.8125 0 26.8125 0 26.8125 0 26.8125 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 60.6875 0 60.6875 0 60.6875 0 60.6875 0 60.6875 26.8125 60.6875 26.8125 60.6875 26.8125 60.6875 26.8125 0 26.8125 0 26.8125 0 26.8125 0 26.8125 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Times New Roman Regular" FONTSIZE="3" CH="{&quot;color&quot;: &quot;blue&quot;, &quot;size&quot;: &quot;large&quot;, &quot;rotation&quot;: 269.8517172617167, &quot;shape&quot;: &quot;cube&quot;, &quot;3d_coords&quot;: [-1.3705521821975708, 2.0794010162353516, 0.699999988079071], &quot;material&quot;: &quot;rubber&quot;, &quot;pixel_coords&quot;: [269, 88, 12.661545753479004]}, ..."/>
            <trail ALIGN="1" LINESPMode="1"/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="162" YPOS="46" WIDTH="4" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="27" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
    </DOCUMENT>
</SCRIBUSUTF8NEW>


==> img/scheme_object_decoding.sla.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<SCRIBUSUTF8NEW Version="1.4.3.svn">
    <DOCUMENT ANZPAGES="1" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" PRESET="0" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" ORIENTATION="1" PAGESIZE="A4" FIRSTNUM="1" BOOK="0" AUTOSPALTEN="1" ABSTSPALTEN="11" UNITS="0" DFONT="Abyssinica SIL Regular" DSIZE="12" DCOL="1" DGAP="0" TabFill="" TabWidth="36" AUTHOR="" COMMENTS="" KEYWORDS="" PUBLISHER="" DOCDATE="" DOCTYPE="" DOCFORMAT="" DOCIDENT="" DOCSOURCE="" DOCLANGINFO="" DOCRELATION="" DOCCOVER="" DOCRIGHTS="" DOCCONTRIB="" TITLE="" SUBJECT="" VHOCH="33" VHOCHSC="66" VTIEF="33" VTIEFSC="66" VKAPIT="75" BASEGRID="5" BASEO="0" AUTOL="20" UnderlinePos="-1" UnderlineWidth="-1" StrikeThruPos="-1" StrikeThruWidth="-1" GROUPC="1" HCMS="0" DPSo="0" DPSFo="0" DPuse="0" DPgam="0" DPbla="1" DPMo="CineonLog M " DPPr="Fogra27L CMYK Coated Press" DPIn="CineonLog M " DPInCMYK="Fogra27L CMYK Coated Press" DPIn2="CineonLog M " DPIn3="Fogra27L CMYK Coated Press" DISc="1" DIIm="0" ALAYER="0" LANGUAGE="English" MINWORDLEN="3" HYCOUNT="2" AUTOMATIC="1" AUTOCHECK="0" GUIDELOCK="0" SnapToGuides="0" SnapToGrid="0" MINGRID="10" MAJGRID="10" SHOWGRID="0" SHOWGUIDES="0" showcolborders="1" SHOWFRAME="0" SHOWLAYERM="0" SHOWMARGIN="0" SHOWBASE="0" SHOWPICT="1" SHOWControl="0" SHOWLINK="0" rulerMode="0" showrulers="0" showBleed="0" rulerXoffset="100" rulerYoffset="20" GuideRad="10" GRAB="4" POLYC="4" POLYF="0.707" POLYR="0" POLYCUR="0" POLYFD="0" POLYS="0" AutoSave="1" AutoSaveTime="600000" ScratchBottom="20" ScratchLeft="100" ScratchRight="100" ScratchTop="20" GapHorizontal="0" GapVertical="40" StartArrow="0" EndArrow="0" PEN="Black" BRUSH="None" PENLINE="Black" PENTEXT="Black" StrokeText="Black" TextBackGround="None" TextLineColor="None" TextBackGroundShade="100" TextLineShade="100" TextPenShade="100" TextStrokeShade="100" STIL="1" STILLINE="1" WIDTH="1" WIDTHLINE="1" PENSHADE="100" LINESHADE="100" BRUSHSHADE="100" MAGMIN="10" MAGMAX="3200" MAGSTEP="200" CPICT="None" PICTSHADE="100" PICTSCX="1" PICTSCY="1" PSCALE="1" PASPECT="1" EmbeddedPath="0" HalfRes="1" dispX="10" dispY="10" constrain="15" MINORC="#aa0000" MAJORC="#aa0000" GuideC="#000080" BaseC="#c0c0c0" GuideZ="10" BACKG="1" PAGEC="#ffffff" MARGC="#0000ff" RANDF="0" currentProfile="PostScript">
        <CheckProfile Name="PDF 1.3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.4" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.5" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF/X-3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="1" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PostScript" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <COLOR NAME="Black" CMYK="#000000ff" Spot="0" Register="0"/>
        <COLOR NAME="Blue" RGB="#0000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cool Black" CMYK="#990000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cyan" CMYK="#ff000000" Spot="0" Register="0"/>
        <COLOR NAME="FromEPS#00000070" CMYK="#00000070" Spot="0" Register="0"/>
        <COLOR NAME="Green" RGB="#00ff00" Spot="0" Register="0"/>
        <COLOR NAME="Grey58" RGB="#949494" Spot="0" Register="0"/>
        <COLOR NAME="Magenta" CMYK="#00ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Red" RGB="#ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Registration" CMYK="#ffffffff" Spot="0" Register="1"/>
        <COLOR NAME="Rich Black" CMYK="#996666ff" Spot="0" Register="0"/>
        <COLOR NAME="Snow2" RGB="#eee9e9" Spot="0" Register="0"/>
        <COLOR NAME="Snow4" RGB="#8b8989" Spot="0" Register="0"/>
        <COLOR NAME="Warm Black" CMYK="#00994cff" Spot="0" Register="0"/>
        <COLOR NAME="White" CMYK="#00000000" Spot="0" Register="0"/>
        <COLOR NAME="Yellow" CMYK="#0000ff00" Spot="0" Register="0"/>
        <HYPHEN/>
        <STYLE NAME="Default Paragraph Style" ALIGN="0" LINESPMode="0" LINESP="15" INDENT="0" RMARGIN="0" FIRST="0" VOR="0" NACH="0" DROP="0" DROPLIN="2" DROPDIST="0"/>
        <CHARSTYLE CNAME="Default Character Style" FONT="Abyssinica SIL Regular" FONTSIZE="12" FEATURES="inherit" FCOLOR="Black" FSHADE="100" SCOLOR="Black" SSHADE="100" TXTSHX="5" TXTSHY="-5" TXTOUT="1" TXTULP="-0.1" TXTULW="-0.1" TXTSTP="-0.1" TXTSTW="-0.1" SCALEH="100" SCALEV="100" BASEO="0" KERN="0" LANGUAGE="English"/>
        <LAYERS NUMMER="0" LEVEL="0" NAME="Background" SICHTBAR="1" DRUCKEN="1" EDIT="1" FLOW="1" TRANS="1" BLEND="0" OUTL="0" LAYERC="#000000"/>
        <Printer firstUse="1" toFile="1" useAltPrintCommand="1" outputSeparations="1" useSpotColors="0" useColor="0" mirrorH="0" mirrorV="0" useICC="0" doGCR="0" doClip="0" setDevParam="0" useDocBleeds="0" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" includePDFMarks="0" PSLevel="3" PDLanguage="3" markOffset="6.94181282764193e-310" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" printer="" filename="" separationName="" printerCommand=""/>
        <PDF firstUse="0" Thumbnails="0" Articles="0" Bookmarks="0" Compress="1" CMethod="0" Quality="0" MirrorH="0" MirrorV="0" Clip="0" RotateDeg="0" PresentMode="0" RecalcPic="0" Grayscale="0" RGBMode="1" UseProfiles="0" UseProfiles2="0" Binding="0" PicRes="300" Resolution="300" Version="14" Intent="1" Intent2="0" SolidP="CineonLog M " ImageP="CineonLog M " PrintP="Fogra27L CMYK Coated Press" InfoString="" BTop="0" BLeft="0" BRight="0" BBottom="0" useDocBleeds="1" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" docInfoMarks="0" markOffset="0" ImagePr="0" PassOwner="" PassUser="" Permissions="-4" Encrypt="0" UseLayers="0" UseLpi="0" UseSpotColors="1" doMultiFile="0" displayBookmarks="0" displayFullscreen="0" displayLayers="0" displayThumbs="0" hideMenuBar="0" hideToolBar="0" fitWindow="0" PageLayout="0" openAction="">
            <Fonts Name="Abyssinica SIL Regular"/>
            <Effekte pageEffectDuration="1" pageViewDuration="1" effectType="0" Dm="0" M="0" Di="0"/>
            <LPI Color="" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Black" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Cyan" Frequency="133" Angle="105" SpotFunction="3"/>
            <LPI Color="Magenta" Frequency="133" Angle="75" SpotFunction="3"/>
            <LPI Color="Yellow" Frequency="133" Angle="90" SpotFunction="3"/>
        </PDF>
        <DocItemAttributes/>
        <TablesOfContents/>
        <PageSets>
            <Set Name="Single Page" FirstPage="0" Rows="1" Columns="1"/>
            <Set Name="Double Sided" FirstPage="1" Rows="1" Columns="2">
                <PageNames Name="Left Page"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="3-Fold" FirstPage="0" Rows="1" Columns="3">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="4-Fold" FirstPage="0" Rows="1" Columns="4">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle Left"/>
                <PageNames Name="Middle Right"/>
                <PageNames Name="Right Page"/>
            </Set>
        </PageSets>
        <Sections>
            <Section Number="0" Name="0" From="0" To="0" Type="Type_1_2_3" Start="1" Reversed="0" Active="1"/>
        </Sections>
        <MASTERPAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="Normal" MNAM="" Size="A4" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="370" PAGEHEIGHT="110" BORDERLEFT="38" BORDERRIGHT="0" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="" MNAM="Normal" Size="Custom" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="102" YPOS="31.0000000000001" WIDTH="30" HEIGHT="40.7462686567164" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.447761194029851" LOCALSCY="0.447761194029851" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object1.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 40.7463 30 40.7463 30 40.7463 30 40.7463 0 40.7463 0 40.7463 0 40.7463 0 40.7463 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 40.7463 30 40.7463 30 40.7463 30 40.7463 0 40.7463 0 40.7463 0 40.7463 0 40.7463 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="185" YPOS="24" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="183" YPOS="22" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="183" YPOS="28" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="Attribute"/>
            <para/>
            <ITEXT CH="extraction"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="262" YPOS="28" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_a\textbf{O}^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="161" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="266" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="112" YPOS="28" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_d\textbf{O}^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="112" YPOS="45" WIDTH="30" HEIGHT="37.9310344827586" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.344827586206897" LOCALSCY="0.344827586206897" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object2.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 37.931 30 37.931 30 37.931 30 37.931 0 37.931 0 37.931 0 37.931 0 37.931 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 37.931 30 37.931 30 37.931 30 37.931 0 37.931 0 37.931 0 37.931 0 37.931 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="122" YPOS="57" WIDTH="30" HEIGHT="31.0526315789473" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.526315789473684" LOCALSCY="0.526315789473684" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object3.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 31.0526 30 31.0526 30 31.0526 30 31.0526 0 31.0526 0 31.0526 0 31.0526 0 31.0526 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 31.0526 30 31.0526 30 31.0526 30 31.0526 0 31.0526 0 31.0526 0 31.0526 0 31.0526 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="132" YPOS="71" WIDTH="30" HEIGHT="29.620253164557" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.379746835443038" LOCALSCY="0.379746835443038" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object4.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 29.6203 30 29.6203 30 29.6203 30 29.6203 0 29.6203 0 29.6203 0 29.6203 0 29.6203 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 29.6203 30 29.6203 30 29.6203 30 29.6203 0 29.6203 0 29.6203 0 29.6203 0 29.6203 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="142" YPOS="85" WIDTH="30" HEIGHT="29.5652173913044" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.434782608695652" LOCALSCY="0.434782608695652" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object5.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 29.5652 30 29.5652 30 29.5652 30 29.5652 0 29.5652 0 29.5652 0 29.5652 0 29.5652 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 29.5652 30 29.5652 30 29.5652 30 29.5652 0 29.5652 0 29.5652 0 29.5652 0 29.5652 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="152" YPOS="100" WIDTH="30" HEIGHT="29.4827586206897" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.517241379310345" LOCALSCY="0.517241379310345" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_object6.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 29.4828 30 29.4828 30 29.4828 30 29.4828 0 29.4828 0 29.4828 0 29.4828 0 29.4828 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 30 0 30 0 30 0 30 0 30 29.4828 30 29.4828 30 29.4828 30 29.4828 0 29.4828 0 29.4828 0 29.4828 0 29.4828 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="202.732050807569" YPOS="57.6025403784438" WIDTH="200" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 200 0 200 0 200 0 200 0 200 20 200 20 200 20 200 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 200 0 200 0 200 0 200 0 200 20 200 20 200 20 200 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$&lt; c^t_0,  m^t_0, s^t_0, f^t_0, x^t_0, y^t_0 &gt;$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="293.709355338635" YPOS="98.148293553917" WIDTH="21.375" HEIGHT="8.625" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="..."/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="335" YPOS="24" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="333" YPOS="22" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="333" YPOS="28" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="Attribute"/>
            <para/>
            <ITEXT CH="embedding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="414" YPOS="28" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_e\textbf{O}^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="416" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="311" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="202.7320508" YPOS="75.60254038" WIDTH="200" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 200 0 200 0 200 0 200 0 200 20 200 20 200 20 200 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 200 0 200 0 200 0 200 0 200 20 200 20 200 20 200 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$&lt; c^t_1,  m^t_1, s^t_1, f^t_1, x^t_1, y^t_1 &gt;$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="202.7320508" YPOS="103.60254038" WIDTH="200" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 200 0 200 0 200 0 200 0 200 20 200 20 200 20 200 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 200 0 200 0 200 0 200 0 200 20 200 20 200 20 200 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$&lt; c^t_5,  m^t_5, s^t_5, f^t_5, x^t_5, y^t_5 &gt;$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="418" YPOS="48" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="421" YPOS="51" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="424" YPOS="54" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="427" YPOS="57" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.2" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="430" YPOS="60" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
    </DOCUMENT>
</SCRIBUSUTF8NEW>


==> img/scheme_object_detection.sla.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<SCRIBUSUTF8NEW Version="1.4.3.svn">
    <DOCUMENT ANZPAGES="1" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" PRESET="0" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" ORIENTATION="1" PAGESIZE="A4" FIRSTNUM="1" BOOK="0" AUTOSPALTEN="1" ABSTSPALTEN="11" UNITS="0" DFONT="Abyssinica SIL Regular" DSIZE="12" DCOL="1" DGAP="0" TabFill="" TabWidth="36" AUTHOR="" COMMENTS="" KEYWORDS="" PUBLISHER="" DOCDATE="" DOCTYPE="" DOCFORMAT="" DOCIDENT="" DOCSOURCE="" DOCLANGINFO="" DOCRELATION="" DOCCOVER="" DOCRIGHTS="" DOCCONTRIB="" TITLE="" SUBJECT="" VHOCH="33" VHOCHSC="66" VTIEF="33" VTIEFSC="66" VKAPIT="75" BASEGRID="5" BASEO="0" AUTOL="20" UnderlinePos="-1" UnderlineWidth="-1" StrikeThruPos="-1" StrikeThruWidth="-1" GROUPC="2" HCMS="0" DPSo="0" DPSFo="0" DPuse="0" DPgam="0" DPbla="1" DPMo="CineonLog M " DPPr="Fogra27L CMYK Coated Press" DPIn="CineonLog M " DPInCMYK="Fogra27L CMYK Coated Press" DPIn2="CineonLog M " DPIn3="Fogra27L CMYK Coated Press" DISc="1" DIIm="0" ALAYER="0" LANGUAGE="English" MINWORDLEN="3" HYCOUNT="2" AUTOMATIC="1" AUTOCHECK="0" GUIDELOCK="0" SnapToGuides="0" SnapToGrid="0" MINGRID="10" MAJGRID="10" SHOWGRID="0" SHOWGUIDES="0" showcolborders="1" SHOWFRAME="0" SHOWLAYERM="0" SHOWMARGIN="0" SHOWBASE="0" SHOWPICT="1" SHOWControl="0" SHOWLINK="0" rulerMode="0" showrulers="0" showBleed="0" rulerXoffset="100" rulerYoffset="20" GuideRad="10" GRAB="4" POLYC="4" POLYF="0.707" POLYR="0" POLYCUR="0" POLYFD="0" POLYS="0" AutoSave="1" AutoSaveTime="600000" ScratchBottom="20" ScratchLeft="100" ScratchRight="100" ScratchTop="20" GapHorizontal="0" GapVertical="40" StartArrow="0" EndArrow="0" PEN="Black" BRUSH="None" PENLINE="Black" PENTEXT="Black" StrokeText="Black" TextBackGround="None" TextLineColor="None" TextBackGroundShade="100" TextLineShade="100" TextPenShade="100" TextStrokeShade="100" STIL="1" STILLINE="1" WIDTH="1" WIDTHLINE="1" PENSHADE="100" LINESHADE="100" BRUSHSHADE="100" MAGMIN="10" MAGMAX="3200" MAGSTEP="200" CPICT="None" PICTSHADE="100" PICTSCX="1" PICTSCY="1" PSCALE="1" PASPECT="1" EmbeddedPath="0" HalfRes="1" dispX="10" dispY="10" constrain="15" MINORC="#aa0000" MAJORC="#aa0000" GuideC="#000080" BaseC="#c0c0c0" GuideZ="10" BACKG="1" PAGEC="#ffffff" MARGC="#0000ff" RANDF="0" currentProfile="PostScript">
        <CheckProfile Name="PDF 1.3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.4" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.5" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF/X-3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="1" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PostScript" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <COLOR NAME="Black" CMYK="#000000ff" Spot="0" Register="0"/>
        <COLOR NAME="Blue" RGB="#0000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cool Black" CMYK="#990000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cyan" CMYK="#ff000000" Spot="0" Register="0"/>
        <COLOR NAME="FromEPS#00000070" CMYK="#00000070" Spot="0" Register="0"/>
        <COLOR NAME="Green" RGB="#00ff00" Spot="0" Register="0"/>
        <COLOR NAME="Grey58" RGB="#949494" Spot="0" Register="0"/>
        <COLOR NAME="Magenta" CMYK="#00ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Red" RGB="#ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Registration" CMYK="#ffffffff" Spot="0" Register="1"/>
        <COLOR NAME="Rich Black" CMYK="#996666ff" Spot="0" Register="0"/>
        <COLOR NAME="Snow2" RGB="#eee9e9" Spot="0" Register="0"/>
        <COLOR NAME="Snow4" RGB="#8b8989" Spot="0" Register="0"/>
        <COLOR NAME="Warm Black" CMYK="#00994cff" Spot="0" Register="0"/>
        <COLOR NAME="White" CMYK="#00000000" Spot="0" Register="0"/>
        <COLOR NAME="Yellow" CMYK="#0000ff00" Spot="0" Register="0"/>
        <HYPHEN/>
        <STYLE NAME="Default Paragraph Style" DefaultStyle="1" ALIGN="0" LINESPMode="0" LINESP="15" INDENT="0" RMARGIN="0" FIRST="0" VOR="0" NACH="0" DROP="0" DROPLIN="2" DROPDIST="0"/>
        <CHARSTYLE CNAME="Default Character Style" DefaultStyle="1" FONT="Abyssinica SIL Regular" FONTSIZE="12" FEATURES="inherit" FCOLOR="Black" FSHADE="100" SCOLOR="Black" SSHADE="100" TXTSHX="5" TXTSHY="-5" TXTOUT="1" TXTULP="-0.1" TXTULW="-0.1" TXTSTP="-0.1" TXTSTW="-0.1" SCALEH="100" SCALEV="100" BASEO="0" KERN="0" LANGUAGE="English"/>
        <LAYERS NUMMER="0" LEVEL="0" NAME="Background" SICHTBAR="1" DRUCKEN="1" EDIT="1" FLOW="1" TRANS="1" BLEND="0" OUTL="0" LAYERC="#000000"/>
        <Printer firstUse="1" toFile="1" useAltPrintCommand="1" outputSeparations="1" useSpotColors="0" useColor="0" mirrorH="0" mirrorV="0" useICC="0" doGCR="0" doClip="0" setDevParam="0" useDocBleeds="0" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" includePDFMarks="0" PSLevel="3" PDLanguage="3" markOffset="6.94181282764193e-310" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" printer="" filename="" separationName="" printerCommand=""/>
        <PDF firstUse="0" Thumbnails="0" Articles="0" Bookmarks="0" Compress="1" CMethod="0" Quality="0" MirrorH="0" MirrorV="0" Clip="0" RotateDeg="0" PresentMode="0" RecalcPic="0" Grayscale="0" RGBMode="1" UseProfiles="0" UseProfiles2="0" Binding="0" PicRes="300" Resolution="300" Version="14" Intent="1" Intent2="0" SolidP="CineonLog M " ImageP="CineonLog M " PrintP="Fogra27L CMYK Coated Press" InfoString="" BTop="0" BLeft="0" BRight="0" BBottom="0" useDocBleeds="1" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" docInfoMarks="0" markOffset="0" ImagePr="0" PassOwner="" PassUser="" Permissions="-4" Encrypt="0" UseLayers="0" UseLpi="0" UseSpotColors="1" doMultiFile="0" displayBookmarks="0" displayFullscreen="0" displayLayers="0" displayThumbs="0" hideMenuBar="0" hideToolBar="0" fitWindow="0" PageLayout="0" openAction="">
            <Fonts Name="Abyssinica SIL Regular"/>
            <Effekte pageEffectDuration="1" pageViewDuration="1" effectType="0" Dm="0" M="0" Di="0"/>
            <LPI Color="" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Black" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Cyan" Frequency="133" Angle="105" SpotFunction="3"/>
            <LPI Color="Magenta" Frequency="133" Angle="75" SpotFunction="3"/>
            <LPI Color="Yellow" Frequency="133" Angle="90" SpotFunction="3"/>
        </PDF>
        <DocItemAttributes/>
        <TablesOfContents/>
        <PageSets>
            <Set Name="Single Page" FirstPage="0" Rows="1" Columns="1"/>
            <Set Name="Double Sided" FirstPage="1" Rows="1" Columns="2">
                <PageNames Name="Left Page"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="3-Fold" FirstPage="0" Rows="1" Columns="3">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="4-Fold" FirstPage="0" Rows="1" Columns="4">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle Left"/>
                <PageNames Name="Middle Right"/>
                <PageNames Name="Right Page"/>
            </Set>
        </PageSets>
        <Sections>
            <Section Number="0" Name="0" From="0" To="0" Type="Type_1_2_3" Start="1" Reversed="0" Active="1"/>
        </Sections>
        <MASTERPAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="Normal" MNAM="" Size="A4" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="230" PAGEHEIGHT="70" BORDERLEFT="38" BORDERRIGHT="0" BORDERTOP="30" BORDERBOTTOM="40" NUM="0" NAM="" MNAM="Normal" Size="Custom" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="102" YPOS="48.0000000000001" WIDTH="60" HEIGHT="40" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.125" LOCALSCY="0.125" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 60 0 60 0 60 0 60 0 60 40 60 40 60 40 60 40 0 40 0 40 0 40 0 40 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 60 0 60 0 60 0 60 0 60 40 60 40 60 40 60 40 0 40 0 40 0 40 0 40 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="2" XPOS="267" YPOS="48" WIDTH="60" HEIGHT="40" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="0.0920245398773006" LOCALSCY="0.0920245398773006" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="0" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="clevr_train_000000_od.png" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="0" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 60 0 60 0 60 0 60 0 60 40 60 40 60 40 60 40 0 40 0 40 0 40 0 40 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 60 0 60 0 60 0 60 0 60 40 60 40 60 40 60 40 0 40 0 40 0 40 0 40 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="175" YPOS="25" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="173" YPOS="23" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="173" YPOS="29" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="10" CH="Object"/>
            <para/>
            <ITEXT CH="detection"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="102" YPOS="27" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$I^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="141" YPOS="38" WIDTH="23.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="256" YPOS="38" WIDTH="23.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="264" YPOS="30" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_d\textbf{O}^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="181.5" YPOS="40.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="187.5" YPOS="40.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="181.453125" YPOS="41.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="187.453125" YPOS="41.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="187.453125" YPOS="41.09375" WIDTH="11.6943496" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="138.9004937" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="181.453125" YPOS="41.09375" WIDTH="11.62821276" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="41.07728711" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="177" YPOS="50" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="183" YPOS="50" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="189" YPOS="50" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="180" YPOS="43" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="186" YPOS="43" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
    </DOCUMENT>
</SCRIBUSUTF8NEW>


==> img/scheme_question_encoding.sla.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<SCRIBUSUTF8NEW Version="1.4.3.svn">
    <DOCUMENT ANZPAGES="1" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" PRESET="0" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" ORIENTATION="1" PAGESIZE="A4" FIRSTNUM="1" BOOK="0" AUTOSPALTEN="1" ABSTSPALTEN="11" UNITS="0" DFONT="Abyssinica SIL Regular" DSIZE="12" DCOL="1" DGAP="0" TabFill="" TabWidth="36" AUTHOR="" COMMENTS="" KEYWORDS="" PUBLISHER="" DOCDATE="" DOCTYPE="" DOCFORMAT="" DOCIDENT="" DOCSOURCE="" DOCLANGINFO="" DOCRELATION="" DOCCOVER="" DOCRIGHTS="" DOCCONTRIB="" TITLE="" SUBJECT="" VHOCH="33" VHOCHSC="66" VTIEF="33" VTIEFSC="66" VKAPIT="75" BASEGRID="5" BASEO="0" AUTOL="20" UnderlinePos="-1" UnderlineWidth="-1" StrikeThruPos="-1" StrikeThruWidth="-1" GROUPC="3" HCMS="0" DPSo="0" DPSFo="0" DPuse="0" DPgam="0" DPbla="1" DPMo="CineonLog M " DPPr="Fogra27L CMYK Coated Press" DPIn="CineonLog M " DPInCMYK="Fogra27L CMYK Coated Press" DPIn2="CineonLog M " DPIn3="Fogra27L CMYK Coated Press" DISc="1" DIIm="0" ALAYER="0" LANGUAGE="English" MINWORDLEN="3" HYCOUNT="2" AUTOMATIC="1" AUTOCHECK="0" GUIDELOCK="0" SnapToGuides="0" SnapToGrid="0" MINGRID="10" MAJGRID="10" SHOWGRID="0" SHOWGUIDES="0" showcolborders="1" SHOWFRAME="0" SHOWLAYERM="0" SHOWMARGIN="0" SHOWBASE="0" SHOWPICT="1" SHOWControl="0" SHOWLINK="0" rulerMode="0" showrulers="0" showBleed="0" rulerXoffset="100" rulerYoffset="20" GuideRad="10" GRAB="4" POLYC="4" POLYF="0.707" POLYR="0" POLYCUR="0" POLYFD="0" POLYS="0" AutoSave="1" AutoSaveTime="600000" ScratchBottom="20" ScratchLeft="100" ScratchRight="100" ScratchTop="20" GapHorizontal="0" GapVertical="40" StartArrow="0" EndArrow="0" PEN="Black" BRUSH="None" PENLINE="Black" PENTEXT="Black" StrokeText="Black" TextBackGround="None" TextLineColor="None" TextBackGroundShade="100" TextLineShade="100" TextPenShade="100" TextStrokeShade="100" STIL="1" STILLINE="1" WIDTH="1" WIDTHLINE="1" PENSHADE="100" LINESHADE="100" BRUSHSHADE="100" MAGMIN="10" MAGMAX="3200" MAGSTEP="200" CPICT="None" PICTSHADE="100" PICTSCX="1" PICTSCY="1" PSCALE="1" PASPECT="1" EmbeddedPath="0" HalfRes="1" dispX="10" dispY="10" constrain="15" MINORC="#aa0000" MAJORC="#aa0000" GuideC="#000080" BaseC="#c0c0c0" GuideZ="10" BACKG="1" PAGEC="#ffffff" MARGC="#0000ff" RANDF="0" currentProfile="PostScript">
        <CheckProfile Name="PDF 1.3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.4" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.5" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF/X-3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="1" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PostScript" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <COLOR NAME="Black" CMYK="#000000ff" Spot="0" Register="0"/>
        <COLOR NAME="Blue" RGB="#0000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cool Black" CMYK="#990000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cyan" CMYK="#ff000000" Spot="0" Register="0"/>
        <COLOR NAME="FromEPS#00000070" CMYK="#00000070" Spot="0" Register="0"/>
        <COLOR NAME="Green" RGB="#00ff00" Spot="0" Register="0"/>
        <COLOR NAME="Grey58" RGB="#949494" Spot="0" Register="0"/>
        <COLOR NAME="Magenta" CMYK="#00ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Red" RGB="#ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Registration" CMYK="#ffffffff" Spot="0" Register="1"/>
        <COLOR NAME="Rich Black" CMYK="#996666ff" Spot="0" Register="0"/>
        <COLOR NAME="Snow2" RGB="#eee9e9" Spot="0" Register="0"/>
        <COLOR NAME="Snow4" RGB="#8b8989" Spot="0" Register="0"/>
        <COLOR NAME="Warm Black" CMYK="#00994cff" Spot="0" Register="0"/>
        <COLOR NAME="White" CMYK="#00000000" Spot="0" Register="0"/>
        <COLOR NAME="Yellow" CMYK="#0000ff00" Spot="0" Register="0"/>
        <HYPHEN/>
        <STYLE NAME="Default Paragraph Style" DefaultStyle="1" ALIGN="0" LINESPMode="0" LINESP="15" INDENT="0" RMARGIN="0" FIRST="0" VOR="0" NACH="0" DROP="0" DROPLIN="2" DROPDIST="0"/>
        <CHARSTYLE CNAME="Default Character Style" DefaultStyle="1" FONT="Abyssinica SIL Regular" FONTSIZE="12" FEATURES="inherit" FCOLOR="Black" FSHADE="100" SCOLOR="Black" SSHADE="100" TXTSHX="5" TXTSHY="-5" TXTOUT="1" TXTULP="-0.1" TXTULW="-0.1" TXTSTP="-0.1" TXTSTW="-0.1" SCALEH="100" SCALEV="100" BASEO="0" KERN="0" LANGUAGE="English"/>
        <LAYERS NUMMER="0" LEVEL="0" NAME="Background" SICHTBAR="1" DRUCKEN="1" EDIT="1" FLOW="1" TRANS="1" BLEND="0" OUTL="0" LAYERC="#000000"/>
        <Printer firstUse="1" toFile="1" useAltPrintCommand="1" outputSeparations="1" useSpotColors="0" useColor="0" mirrorH="0" mirrorV="0" useICC="0" doGCR="0" doClip="0" setDevParam="0" useDocBleeds="0" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" includePDFMarks="0" PSLevel="3" PDLanguage="3" markOffset="6.94181282764193e-310" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" printer="" filename="" separationName="" printerCommand=""/>
        <PDF firstUse="0" Thumbnails="0" Articles="0" Bookmarks="0" Compress="1" CMethod="0" Quality="0" MirrorH="0" MirrorV="0" Clip="0" RotateDeg="0" PresentMode="0" RecalcPic="0" Grayscale="0" RGBMode="1" UseProfiles="0" UseProfiles2="0" Binding="0" PicRes="300" Resolution="300" Version="14" Intent="1" Intent2="0" SolidP="CineonLog M " ImageP="CineonLog M " PrintP="Fogra27L CMYK Coated Press" InfoString="" BTop="0" BLeft="0" BRight="0" BBottom="0" useDocBleeds="1" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" docInfoMarks="0" markOffset="0" ImagePr="0" PassOwner="" PassUser="" Permissions="-4" Encrypt="0" UseLayers="0" UseLpi="0" UseSpotColors="1" doMultiFile="0" displayBookmarks="0" displayFullscreen="0" displayLayers="0" displayThumbs="0" hideMenuBar="0" hideToolBar="0" fitWindow="0" PageLayout="0" openAction="">
            <Fonts Name="Abyssinica SIL Regular"/>
            <Effekte pageEffectDuration="1" pageViewDuration="1" effectType="0" Dm="0" M="0" Di="0"/>
            <LPI Color="" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Black" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Cyan" Frequency="133" Angle="105" SpotFunction="3"/>
            <LPI Color="Magenta" Frequency="133" Angle="75" SpotFunction="3"/>
            <LPI Color="Yellow" Frequency="133" Angle="90" SpotFunction="3"/>
        </PDF>
        <DocItemAttributes/>
        <TablesOfContents/>
        <PageSets>
            <Set Name="Single Page" FirstPage="0" Rows="1" Columns="1"/>
            <Set Name="Double Sided" FirstPage="1" Rows="1" Columns="2">
                <PageNames Name="Left Page"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="3-Fold" FirstPage="0" Rows="1" Columns="3">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="4-Fold" FirstPage="0" Rows="1" Columns="4">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle Left"/>
                <PageNames Name="Middle Right"/>
                <PageNames Name="Right Page"/>
            </Set>
        </PageSets>
        <Sections>
            <Section Number="0" Name="0" From="0" To="0" Type="Type_1_2_3" Start="1" Reversed="0" Active="1"/>
        </Sections>
        <MASTERPAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="Normal" MNAM="" Size="A4" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="340" PAGEHEIGHT="70" BORDERLEFT="38" BORDERRIGHT="0" BORDERTOP="20" BORDERBOTTOM="40" NUM="0" NAM="" MNAM="Normal" Size="Custom" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="153" YPOS="24" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="151" YPOS="22" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="151" YPOS="28" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="10" CH="Word"/>
            <para/>
            <ITEXT CH="embedding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="229" YPOS="28" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_w\textbf{Q}^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="129" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="234" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="83" YPOS="28" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$\textbf{Q}^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="303" YPOS="24" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="301" YPOS="22" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="301" YPOS="28" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="Sequence"/>
            <para/>
            <ITEXT CH="embedding"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="382" YPOS="28" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_s\textbf{Q}^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="384" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="279" YPOS="37" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="94" YPOS="45" WIDTH="40" HEIGHT="50" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 50 40 50 40 50 40 50 0 50 0 50 0 50 0 50 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 50 40 50 40 50 40 50 0 50 0 50 0 50 0 50 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="10" CH="What"/>
            <para/>
            <ITEXT CH="is"/>
            <para/>
            <ITEXT CH="the"/>
            <para/>
            <ITEXT CH="object"/>
            <para/>
            <ITEXT CH="..."/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="157.5" YPOS="26.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="163.5" YPOS="26.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="157.453125" YPOS="27.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="163.453125" YPOS="27.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="163.453125" YPOS="27.09375" WIDTH="11.6943496" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="138.9004937" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="157.453125" YPOS="27.09375" WIDTH="11.62821276" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="41.07728711" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="153" YPOS="36" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="159" YPOS="36" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="165" YPOS="36" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="156" YPOS="29" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="162" YPOS="29" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="307.5" YPOS="26.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="313.5" YPOS="26.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="307.453125" YPOS="27.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="313.453125" YPOS="27.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="313.453125" YPOS="27.09375" WIDTH="11.6943496" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="138.9004937" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="307.453125" YPOS="27.09375" WIDTH="11.62821276" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="41.07728711" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="303" YPOS="36" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="309" YPOS="36" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="315" YPOS="36" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="306" YPOS="29" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="312" YPOS="29" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="247" YPOS="48" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="250" YPOS="51" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="253" YPOS="54" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="256" YPOS="57" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.2" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="259" YPOS="60" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Yellow" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="387" YPOS="48" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="390" YPOS="51" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="393" YPOS="54" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.4" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="396" YPOS="57" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.2" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="399" YPOS="60" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
    </DOCUMENT>
</SCRIBUSUTF8NEW>


==> img/scheme_semantic_embedding.sla.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<SCRIBUSUTF8NEW Version="1.4.3.svn">
    <DOCUMENT ANZPAGES="1" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" PRESET="0" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" ORIENTATION="1" PAGESIZE="A4" FIRSTNUM="1" BOOK="0" AUTOSPALTEN="1" ABSTSPALTEN="11" UNITS="0" DFONT="Abyssinica SIL Regular" DSIZE="12" DCOL="1" DGAP="0" TabFill="" TabWidth="36" AUTHOR="" COMMENTS="" KEYWORDS="" PUBLISHER="" DOCDATE="" DOCTYPE="" DOCFORMAT="" DOCIDENT="" DOCSOURCE="" DOCLANGINFO="" DOCRELATION="" DOCCOVER="" DOCRIGHTS="" DOCCONTRIB="" TITLE="" SUBJECT="" VHOCH="33" VHOCHSC="66" VTIEF="33" VTIEFSC="66" VKAPIT="75" BASEGRID="5" BASEO="0" AUTOL="20" UnderlinePos="-1" UnderlineWidth="-1" StrikeThruPos="-1" StrikeThruWidth="-1" GROUPC="4" HCMS="0" DPSo="0" DPSFo="0" DPuse="0" DPgam="0" DPbla="1" DPMo="CineonLog M " DPPr="Fogra27L CMYK Coated Press" DPIn="CineonLog M " DPInCMYK="Fogra27L CMYK Coated Press" DPIn2="CineonLog M " DPIn3="Fogra27L CMYK Coated Press" DISc="1" DIIm="0" ALAYER="0" LANGUAGE="English" MINWORDLEN="3" HYCOUNT="2" AUTOMATIC="1" AUTOCHECK="0" GUIDELOCK="0" SnapToGuides="0" SnapToGrid="0" MINGRID="10" MAJGRID="10" SHOWGRID="0" SHOWGUIDES="0" showcolborders="1" SHOWFRAME="0" SHOWLAYERM="0" SHOWMARGIN="0" SHOWBASE="0" SHOWPICT="1" SHOWControl="0" SHOWLINK="0" rulerMode="0" showrulers="0" showBleed="0" rulerXoffset="100" rulerYoffset="20" GuideRad="10" GRAB="4" POLYC="4" POLYF="0.707" POLYR="0" POLYCUR="0" POLYFD="0" POLYS="0" AutoSave="1" AutoSaveTime="600000" ScratchBottom="20" ScratchLeft="100" ScratchRight="100" ScratchTop="20" GapHorizontal="0" GapVertical="40" StartArrow="0" EndArrow="0" PEN="Black" BRUSH="None" PENLINE="Black" PENTEXT="Black" StrokeText="Black" TextBackGround="None" TextLineColor="None" TextBackGroundShade="100" TextLineShade="100" TextPenShade="100" TextStrokeShade="100" STIL="1" STILLINE="1" WIDTH="1" WIDTHLINE="1" PENSHADE="100" LINESHADE="100" BRUSHSHADE="100" MAGMIN="10" MAGMAX="3200" MAGSTEP="200" CPICT="None" PICTSHADE="100" PICTSCX="1" PICTSCY="1" PSCALE="1" PASPECT="1" EmbeddedPath="0" HalfRes="1" dispX="10" dispY="10" constrain="15" MINORC="#aa0000" MAJORC="#aa0000" GuideC="#000080" BaseC="#c0c0c0" GuideZ="10" BACKG="1" PAGEC="#ffffff" MARGC="#0000ff" RANDF="0" currentProfile="PostScript">
        <CheckProfile Name="PDF 1.3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.4" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF 1.5" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="0" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PDF/X-3" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="1" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <CheckProfile Name="PostScript" ignoreErrors="0" autoCheck="1" checkGlyphs="1" checkOrphans="1" checkOverflow="1" checkPictures="1" checkResolution="1" checkTransparency="1" minResolution="144" maxResolution="2400" checkAnnotations="0" checkRasterPDF="1" checkForGIF="1" ignoreOffLayers="0" checkOffConflictLayers="0"/>
        <COLOR NAME="Black" CMYK="#000000ff" Spot="0" Register="0"/>
        <COLOR NAME="Blue" RGB="#0000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cool Black" CMYK="#990000ff" Spot="0" Register="0"/>
        <COLOR NAME="Cyan" CMYK="#ff000000" Spot="0" Register="0"/>
        <COLOR NAME="FromEPS#00000070" CMYK="#00000070" Spot="0" Register="0"/>
        <COLOR NAME="Green" RGB="#00ff00" Spot="0" Register="0"/>
        <COLOR NAME="Grey58" RGB="#949494" Spot="0" Register="0"/>
        <COLOR NAME="Magenta" CMYK="#00ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Red" RGB="#ff0000" Spot="0" Register="0"/>
        <COLOR NAME="Registration" CMYK="#ffffffff" Spot="0" Register="1"/>
        <COLOR NAME="Rich Black" CMYK="#996666ff" Spot="0" Register="0"/>
        <COLOR NAME="Snow2" RGB="#eee9e9" Spot="0" Register="0"/>
        <COLOR NAME="Snow4" RGB="#8b8989" Spot="0" Register="0"/>
        <COLOR NAME="Warm Black" CMYK="#00994cff" Spot="0" Register="0"/>
        <COLOR NAME="White" CMYK="#00000000" Spot="0" Register="0"/>
        <COLOR NAME="Yellow" CMYK="#0000ff00" Spot="0" Register="0"/>
        <HYPHEN/>
        <STYLE NAME="Default Paragraph Style" DefaultStyle="1" ALIGN="0" LINESPMode="0" LINESP="15" INDENT="0" RMARGIN="0" FIRST="0" VOR="0" NACH="0" DROP="0" DROPLIN="2" DROPDIST="0"/>
        <CHARSTYLE CNAME="Default Character Style" DefaultStyle="1" FONT="Abyssinica SIL Regular" FONTSIZE="12" FEATURES="inherit" FCOLOR="Black" FSHADE="100" SCOLOR="Black" SSHADE="100" TXTSHX="5" TXTSHY="-5" TXTOUT="1" TXTULP="-0.1" TXTULW="-0.1" TXTSTP="-0.1" TXTSTW="-0.1" SCALEH="100" SCALEV="100" BASEO="0" KERN="0" LANGUAGE="English"/>
        <LAYERS NUMMER="0" LEVEL="0" NAME="Background" SICHTBAR="1" DRUCKEN="1" EDIT="1" FLOW="1" TRANS="1" BLEND="0" OUTL="0" LAYERC="#000000"/>
        <Printer firstUse="1" toFile="1" useAltPrintCommand="1" outputSeparations="1" useSpotColors="0" useColor="0" mirrorH="0" mirrorV="0" useICC="0" doGCR="0" doClip="0" setDevParam="0" useDocBleeds="0" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" includePDFMarks="0" PSLevel="3" PDLanguage="3" markOffset="6.94181282764193e-310" BleedTop="0" BleedLeft="0" BleedRight="0" BleedBottom="0" printer="" filename="" separationName="" printerCommand=""/>
        <PDF firstUse="0" Thumbnails="0" Articles="0" Bookmarks="0" Compress="1" CMethod="0" Quality="0" MirrorH="0" MirrorV="0" Clip="0" RotateDeg="0" PresentMode="0" RecalcPic="0" Grayscale="0" RGBMode="1" UseProfiles="0" UseProfiles2="0" Binding="0" PicRes="300" Resolution="300" Version="14" Intent="1" Intent2="0" SolidP="CineonLog M " ImageP="CineonLog M " PrintP="Fogra27L CMYK Coated Press" InfoString="" BTop="0" BLeft="0" BRight="0" BBottom="0" useDocBleeds="1" cropMarks="0" bleedMarks="0" registrationMarks="0" colorMarks="0" docInfoMarks="0" markOffset="0" ImagePr="0" PassOwner="" PassUser="" Permissions="-4" Encrypt="0" UseLayers="0" UseLpi="0" UseSpotColors="1" doMultiFile="0" displayBookmarks="0" displayFullscreen="0" displayLayers="0" displayThumbs="0" hideMenuBar="0" hideToolBar="0" fitWindow="0" PageLayout="0" openAction="">
            <Fonts Name="Abyssinica SIL Regular"/>
            <Effekte pageEffectDuration="1" pageViewDuration="1" effectType="0" Dm="0" M="0" Di="0"/>
            <LPI Color="" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Black" Frequency="133" Angle="45" SpotFunction="3"/>
            <LPI Color="Cyan" Frequency="133" Angle="105" SpotFunction="3"/>
            <LPI Color="Magenta" Frequency="133" Angle="75" SpotFunction="3"/>
            <LPI Color="Yellow" Frequency="133" Angle="90" SpotFunction="3"/>
        </PDF>
        <DocItemAttributes/>
        <TablesOfContents/>
        <PageSets>
            <Set Name="Single Page" FirstPage="0" Rows="1" Columns="1"/>
            <Set Name="Double Sided" FirstPage="1" Rows="1" Columns="2">
                <PageNames Name="Left Page"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="3-Fold" FirstPage="0" Rows="1" Columns="3">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle"/>
                <PageNames Name="Right Page"/>
            </Set>
            <Set Name="4-Fold" FirstPage="0" Rows="1" Columns="4">
                <PageNames Name="Left Page"/>
                <PageNames Name="Middle Left"/>
                <PageNames Name="Middle Right"/>
                <PageNames Name="Right Page"/>
            </Set>
        </PageSets>
        <Sections>
            <Section Number="0" Name="0" From="0" To="0" Type="Type_1_2_3" Start="1" Reversed="0" Active="1"/>
        </Sections>
        <MASTERPAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="841.89" PAGEHEIGHT="595.28" BORDERLEFT="40" BORDERRIGHT="40" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="Normal" MNAM="" Size="A4" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGE PAGEXPOS="100" PAGEYPOS="20" PAGEWIDTH="390" PAGEHEIGHT="120" BORDERLEFT="38" BORDERRIGHT="0" BORDERTOP="40" BORDERBOTTOM="40" NUM="0" NAM="" MNAM="Normal" Size="Custom" Orientation="1" LEFT="0" PRESET="0" VerticalGuides="" HorizontalGuides="" AGhorizontalAutoGap="0" AGverticalAutoGap="0" AGhorizontalAutoCount="0" AGverticalAutoCount="0" AGhorizontalAutoRefer="0" AGverticalAutoRefer="0" AGSelection="0 0 0 0"/>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="248" YPOS="30" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="246" YPOS="28" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="246" YPOS="34" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="10" CH="Object relation"/>
            <para/>
            <ITEXT CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="317" YPOS="37" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$r^t_{0,1}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="329" YPOS="43" WIDTH="35.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-315" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="363" YPOS="70" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="361" YPOS="68" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="361" YPOS="74" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="10" CH="Relation"/>
            <para/>
            <ITEXT CH="aggregation"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="91" YPOS="18.9" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_eo^t_0$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="224" YPOS="43" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="139.875" YPOS="92.125" WIDTH="21.375" HEIGHT="8.625" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="..."/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="166" YPOS="17.9" WIDTH="70" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_sq^t_{W-1}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="131" YPOS="18.9" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_eo^t_0$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.5" YPOS="45.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.5" YPOS="45.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.453125" YPOS="46.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.453125" YPOS="46.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.453125" YPOS="46.09375" WIDTH="11.6943496" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="138.9004937" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.453125" YPOS="46.09375" WIDTH="11.62821276" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="41.07728711" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="251" YPOS="55" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="257" YPOS="55" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="263" YPOS="55" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="254" YPOS="48" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="260" YPOS="48" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="248" YPOS="70" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="246" YPOS="68" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="246" YPOS="74" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="10" CH="Object relation"/>
            <para/>
            <ITEXT CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.5" YPOS="85.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.5" YPOS="85.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.453125" YPOS="86.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.453125" YPOS="86.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.453125" YPOS="86.09375" WIDTH="11.6943496" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="138.9004937" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.453125" YPOS="86.09375" WIDTH="11.62821276" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="41.07728711" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="251" YPOS="95" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="257" YPOS="95" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="263" YPOS="95" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="254" YPOS="88" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="260" YPOS="88" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="248" YPOS="110" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="Snow4" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="246" YPOS="108" WIDTH="80" HEIGHT="30" RADRECT="10" FRTYPE="2" CLIPEDIT="0" PWIDTH="1" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="32" POCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMCO="32" COCOOR="10 0 10 0 70 0 70 0 70 0 75.5228 0 80 10 80 4.47715 80 10 80 10 80 20 80 20 80 20 80 25.5228 70 30 75.5228 30 70 30 70 30 10 30 10 30 10 30 4.47715 30 0 20 0 25.5228 0 20 0 20 0 10 0 10 0 10 0 4.47715 10 0 4.47715 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="246" YPOS="114" WIDTH="80" HEIGHT="25" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LINESP="9" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" IFONT="Abyssinica SIL Regular" ISIZE="10" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 80 0 80 0 80 0 80 0 80 25 80 25 80 25 80 25 0 25 0 25 0 25 0 25 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" ALIGN="1" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT FONT="Abyssinica SIL Regular" FONTSIZE="10" CH="Object relation"/>
            <para/>
            <ITEXT CH="MLP"/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.5" YPOS="125.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.5" YPOS="125.8125" WIDTH="8.838641413" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="110.1648324" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.453125" YPOS="126.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.453125" YPOS="126.09375" WIDTH="8.558635651" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="69.4806828" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="261.453125" YPOS="126.09375" WIDTH="11.6943496" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="138.9004937" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="255.453125" YPOS="126.09375" WIDTH="11.62821276" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="41.07728711" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="251" YPOS="135" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="257" YPOS="135" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="263" YPOS="135" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="254" YPOS="128" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="260" YPOS="128" WIDTH="3" HEIGHT="3" RADRECT="0" FRTYPE="1" CLIPEDIT="0" PWIDTH="0" PCOLOR="White" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-90" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMCO="16" COCOOR="3 1.5 3 2.32846 1.5 3 2.32846 3 1.5 3 0.671573 3 0 1.5 0 2.32846 0 1.5 0 0.671573 1.5 0 0.671573 0 1.5 0 2.32846 0 3 1.5 3 0.671573 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="277.875" YPOS="102.125" WIDTH="21.375" HEIGHT="8.625" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="..."/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="329" YPOS="83" WIDTH="23.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="329" YPOS="123" WIDTH="35.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="-45" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="303" YPOS="62" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$r^t_{0,2}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="4" XPOS="331.875" YPOS="94.125" WIDTH="21.375" HEIGHT="8.625" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 21.375 0 21.375 0 21.375 0 21.375 0 21.375 8.625 21.375 8.625 21.375 8.625 21.375 8.625 0 8.625 0 8.625 0 8.625 0 8.625 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <ITEXT CH="..."/>
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="318" YPOS="113" WIDTH="90" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 90 0 90 0 90 0 90 0 90 20 90 20 90 20 90 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 90 0 90 0 90 0 90 0 90 20 90 20 90 20 90 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$r^t_{N-1,N-2}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="224" YPOS="83" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="224" YPOS="123" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="91" YPOS="60" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_eo^t_0$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="131" YPOS="60" WIDTH="50" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 50 0 50 0 50 0 50 0 50 20 50 20 50 20 50 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_eo^t_1$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="166" YPOS="57.9" WIDTH="70" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_sq^t_{W-1}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="85" YPOS="98" WIDTH="70" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_eo^t_{N-1}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="122" YPOS="98" WIDTH="60" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 60 0 60 0 60 0 60 0 60 20 60 20 60 20 60 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 60 0 60 0 60 0 60 0 60 20 60 20 60 20 60 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_eo^t_{N-1}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="166" YPOS="95.9" WIDTH="70" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 70 0 70 0 70 0 70 0 70 20 70 20 70 20 70 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_sq^t_{W-1}$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="9" XPOS="441" YPOS="72" WIDTH="45" HEIGHT="20" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="0" PCOLOR="None" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="4" LOCALY="-1" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="0" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 45 0 45 0 45 0 45 0 45 20 45 20 45 20 45 20 0 20 0 20 0 20 0 20 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <LATEX ConfigFile="100_latex.xml" DPI="0" USE_PREAMBLE="1">
                <PROPERTY name="additionalheaders" value="\usepackage{amsmath}"/>
                <PROPERTY name="font" value=""/>
                <PROPERTY name="fontsize" value="14pt"/>$_ar^t$</LATEX>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="5" XPOS="444" YPOS="83" WIDTH="13.5" HEIGHT="1" RADRECT="0" FRTYPE="0" CLIPEDIT="0" PWIDTH="1" PCOLOR="None" PCOLOR2="Black" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="0" POCOOR="" NUMCO="0" COCOOR="" NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="2" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <para/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="103" YPOS="39" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="143" YPOS="39" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="103" YPOS="119" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="143" YPOS="79" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.6" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="143" YPOS="119" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="183" YPOS="39" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="103" YPOS="79" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Red" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0.8" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="183" YPOS="79" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="183" YPOS="119" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Green" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
        <PAGEOBJECT OwnPage="0" PTYPE="6" XPOS="445" YPOS="92" WIDTH="40" HEIGHT="8" RADRECT="0" FRTYPE="0" CLIPEDIT="1" PWIDTH="0" PCOLOR="Blue" PCOLOR2="None" COLUMNS="1" COLGAP="0" NAMEDLST="" SHADE="100" SHADE2="100" GRTYP="0" ROT="0" PLINEART="1" PLINEEND="0" PLINEJOIN="0" LOCALSCX="1" LOCALSCY="1" LOCALX="0" LOCALY="0" PICART="1" PLTSHOW="0" BASEOF="0" textPathType="0" textPathFlipped="0" FLIPPEDH="0" FLIPPEDV="0" SCALETYPE="1" RATIO="1" PRINTABLE="1" ANNOTATION="0" ANNAME="" TEXTFLOWMODE="0" TEXTFLOW="0" TEXTFLOW2="0" TEXTFLOW3="0" AUTOTEXT="0" EXTRA="0" TEXTRA="0" BEXTRA="0" REXTRA="0" FLOP="0" PFILE="" PFILE2="" PFILE3="" PRFILE="" EPROF="" IRENDER="1" EMBEDDED="1" LOCK="0" LOCKR="0" REVERS="0" TransValue="0" TransValueS="0" TransBlend="0" TransBlendS="0" isTableItem="0" TopLine="0" LeftLine="0" RightLine="0" BottomLine="0" isGroupControl="0" NUMDASH="0" DASHS="" DASHOFF="0" NUMPO="16" POCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMCO="16" COCOOR="0 0 0 0 40 0 40 0 40 0 40 0 40 8 40 8 40 8 40 8 0 8 0 8 0 8 0 8 0 0 0 0 " NUMGROUP="0" GROUPS="" startArrowIndex="0" endArrowIndex="0" OnMasterPage="" ImageClip="" ImageRes="1" Pagenumber="0" isInline="0" fillRule="1" doOverprint="0" gXpos="0" gYpos="0" gWidth="0" gHeight="0" LAYER="0" BOOKMARK="0" NEXTITEM="-1" BACKITEM="-1">
            <trail/>
            <PageItemAttributes/>
        </PAGEOBJECT>
    </DOCUMENT>
</SCRIBUSUTF8NEW>

